Improving Self-Supervised Learning by Characterizing Idealized Representations

Despite the empirical successes of self-supervised learning (SSL) methods, it is unclear what characteristics of their representations lead to high downstream accuracies. In this work, we characterize properties that SSL representations should ideally satisfy. Specifically, we prove necessary and sufficient conditions such that for any task invariant to given data augmentations, desired probes (e.g., linear or MLP) trained on that representation attain perfect accuracy. These requirements lead to a unifying conceptual framework for improving existing SSL methods and deriving new ones. For contrastive learning, our framework prescribes simple but significant improvements to previous methods such as using asymmetric projection heads. For non-contrastive learning, we use our framework to derive a simple and novel objective. Our resulting SSL algorithms outperform baselines on standard benchmarks, including SwAV+multicrops on linear probing of ImageNet.

==> appendices/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% BEGIN INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
   \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} in \cref{sec:discussion} expanded in \cref{sec:appx:discussion} .
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}.% in \cref{sec:appx:discussion}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
     \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerYes{} in  the paper the main paper we mention the important ones succintly, in \cref{sec:appx:prel:assumptions} we discuss each in detail.
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} in \cref{sec:appx:proofs}.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
   \answerYes{} all the code to reproduce our results can be found at \codeurl{}.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
     \answerYes{} in \cref{sec:appx:reproducability}.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
     \answerYes{} for the TinyImageNet table. We did not for ImageNet due to computational constraints.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{}.
  \item Did you mention the license of the assets?
  \answerNo{}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}.
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}.
\end{enumerate}


\end{enumerate}


==> appendices/insights.tex <==
\paragraph{Effective dimensionality}

\clearpage
\newpage

==> appendices/myths_sec.tex <==
\clearpage
\newpage

==> appendices/proofs.tex <==

First, we will show that the minimal sample size on size to perform all downstream invariant task is at least the number of equivalence classes.
This should not be a surprise as any task that differs only on one equivalent class will also be in $\tasksinv{}$ so one needs to at least see one example per equivalence class to know which is the current task.

\begin{lemma}\label{lemma:min_n_samples}
The required sample size for any discriminative encoder $\p{Z|X} \in \dP{}$ is $\rS{} \geq |\mathcal{X} / \sim|$.
\end{lemma}
\begin{proof}
Suppose that $\rS{} < |\mathcal{X} / \sim|$.
I.e., for any invariant task $Y \in \tasksinv{}$ there exists a dataset $\Dy$ of size $|\Dy| < |\mathcal{X} / \sim|$ s.t. all ERM $\hat{f} \in \eBQ(\Dy)$ is a Bayes predictor $f \in \BQ{}$.
Importantly this means that for any $\Dy$ there is at least one equivalence class $[x]_{miss}$ for which no member of it are in $\Dy$.
As the encoder is discriminative and by \cref{lemma:achieve_0}, we have that for any deterministic function $g$ that is invariant w.r.t. $(\Xc,sim)$ there must exist a function $f \in \Q$ s.t. $f(Z) = g(X)$.
In particular there exists two functions $f,f' \in \Q$ that achieve predict the correct labeling for all representation from coming from examples in $\Dy$ but predict differently on examples coming from the missing equivalence class $[x]_{miss}$.
By construction $f,f' \in \eBQ(\Dy)$ are ERM's but cannot both be actual risk minimizers.
Contradiction.
\end{proof}

\Cref{lemma:min_n_samples} shows that even when the dataset can have different inputs $X$ they need to contain at least one example per equivalence class. 
We now show that this lower bound is achievable by representations that are essentially maximal invariants (or stochastic versions thereof).
Furthermore, any dataset that have at least one single example per equivalence class then ensures that ERM's from these sample efficient encoders are population risk minimizers.

\begin{lemma}[Sample efficient encoders]\label{lemma:sufficient_data}
Let $\p{Z|X} \in \dP{}$ be a discriminative encoder.
Any set $\Sc$ containing an example from each equivalence class is sufficient for $\Q,\tasksinv{},Z$ if the support of the encoder is a maximal invariant, \ie, $\supp{p(Z|x)} = \supp{p(Z|x^+)} \iff x \sim x^+$.
\end{lemma}
\begin{proof}
\begin{itemize}
\item Show that any $D$ with more than an example per equivalence class is redundant, so focus on one per class.
\item Show that for any $D$ with one equivalence per class if you achieve empirical bayes risk you learn how to predict the most likely label perfectly (because discriminative)
\item say that most likely label is a bayes predictor for population task
\item conclude by saying that all empirical bayes predictors predict a population bayes predictor as desired.
\end{itemize}
\end{proof}

Note that when family is unconstrained $\U$ \cref{lemma:sufficient_data} can actually be shown to be an if and only if statement.
For the case of constrained functional essentially any representations s.t. Bayes predictors are cannot distinguish between the support of equivalent examples will be sample efficient. 
As this depends on the task and the Bayes predictors, we only gave the simpler statement of having the same conditional support.

Putting both previous statements together gives directly  \cref{prop:sample_eff_encoder}.

\begin{manualprop}{\ref{prop:sample_eff_encoder}}
Let $\p{Z|X} \in \dP{}$ be a discriminative encoder.
The required sample size is $\rS{} \geq |\mathcal{X} / \sim|$ with equality if  $\supp{p(Z|x)} = \supp{p(Z|x^+)} \iff x \sim x^+$.
\end{manualprop}
\begin{proof}
$\rS{} \geq |\mathcal{X} / \sim|$ due to \cref{lemma:min_n_samples}.
Equality comes from \cref{lemma:sufficient_data}.
\end{proof}


\Cref{prop:sample_eff_support} only concerns the best case dataset (minimal number of samples), but we can easily convert it into a statement about average case dataset (expected number of samples to see) using results from the coupon collector problem.
For simplicity let us only consider tasks that are deterministic labeling of the inputs.
Then expected number of samples (over \iid samples from $\p{X,Y}$) s.t. for any invariant task, all empirical Bayes predictors are population Bayes prediction is simply the expected number of samples before sampling one example per equivalence class.
When the inputs are s.t. that that the equivalence classes are equiprobable.
We know by standard coupon collector results that this expected number scales as $\Theta(|\Xc / \sim| \log |\Xc / \sim|)$, as seen for example in \citet{ross_first_2010}.
In the non-equiprobable case, one can use results from the weighted coupon collector problem.
For example, if the sorted distribution of equivalence class is $\mathbf{p} = (p(M(X)=m_1), \dots, p(M(X)=m_{|\Mc|})$ where $\mathbf{p}_i \leq \mathbf{p}_{i+1}$.
Then the expected number of samples will essentially scale as $\sum_{i=1}^{|\Mc|} \frac{1}{i \cdot \mathbf{p}_i }$ \cite{berenbrink_weighted_2009}.

% \begin{corollary}
% Let $\p{Z|X}$ be an encoder that satisfies the support constraint from \cref{prop:sample_eff_support}.
% Let $X$ and $(\Xc,\sim)$ be s.t. that the probability of each equivalence class is the same, \ie, $p([x]) = p([x'])$ for all $x,x' \in \Xc$.
% Let $Y$
% Then the expected (over sampling from $\p{X,Y}$) number of samples $|\Dy|$ drawn \iid from $\p{X,Y}$ s.t. for any 

% Then the expected (over 

% Let $\Dy$ be a dataset of $\iid$ samples from the joint $\p{X,Y}$
% \end{corollary}

\subsection{Proofs for sample space $\Zc$}


One simple and useful lemma is that considering stochastic encoders does not change the requirements on the sample space.

\begin{lemma}[Deterministic is sufficient]\label{lemma:det_sufficient}
Let $\p{Z|X}$ be an encoder that can be shattered by $\Q$ w.r.t. $(\Xc,\sim)$.
Then there exists a deterministic representation $Z_{det} = e(X)$ that t.v.i. $\Zc_{det} \subseteq \supp{\p{Z}}$ and can be shattered by $\Q$ w.r.t. $(\Xc,\sim)$.
\end{lemma}
\begin{proof}
Suppose that $\p{Z|X}$ is s.t. for any binary labeling $b \in 2^{\Mc}$ there exists $\pred{} \in \Q$ s.t. $f(Z) = b(M(X))$. 
Then one can easily construct a deterministic encoder mapping $x$ to a point in the conditional support, \eg (one of) the mode(s) $e : x \to \argmax_z p(z|X)$,  that would satisfy $f(e(x)) = b(M(X))$.
Clearly the resulting support cannot be larger than the original one and so $\supp{p(Z_{det})} \subseteq \supp{p(Z)}$.
Then let $\Zc_{det} = \supp{p(Z_{det})}$ which concludes the proof.
\end{proof}

First, let us prove that that the the necessity of shattering w.r.t. $\Q,\sim$ is tightly related to the VC dimension of $\Q$.
This should not be surprising given that VC dimension is tightly related to classical shattering, which is itself tightly related to our invariant shattering.

\begin{manualprop}{\ref{prop:VC_dimension}}[Invariant shattering and VC dimension]
There exists a discriminative encoder $\p{Z|X} \in \dP{}$ if and only if the VC dimension of $\Q$ is at least the number of equivalence classes, \ie,  $\op{VC}{\Q} \geq |\mathcal{X} / \sim|$.
\end{manualprop}
\begin{proof}
By \cref{lem:induction}, there exists an encoder that is discriminative $\p{Z|X} \in \dP{}$ if and only if there exists a shattered encoder $\p{Z|X} \in \sP{}$.
Now let us show that shattering if possible if and only if $\op{VC}{\Q} \geq |\mathcal{X} / \sim|$.
As any maximal invariant is a bijection from the quotient set to some $\Mc$, the cardinality of the image of $\Xc$ by $M$ is $|\mathcal{X} / \sim|$.

($\impliedby$) Let $\op{VC}{\Q} \geq |\mathcal{X} / \sim|$, then by definition there exists some set of $|\mathcal{X} / \sim|$ points $\mathcal{D} = \set{z_1,\dots, z_n}$ in $\Zc$ that can be (clasically) shattered by $\Q$.
As $\mathcal{D}$ has cardinality $|\mathcal{X} / \sim|$ there exists a maximal invariant $M(X)$ whose image is $\mathcal{D}$, let $p(Z|X)$ be deterministic with $Z = M(X)$. 
By construction $\mathcal{D}$ can be (clasically) shattered by $\Q$ so for any binary labeling $b \in 2^{\Mc}$ there exists a $\pred{} \in \Q$ s.t. $f(Z) = b(Z)=b(M(X))$, \ie, $p(Z|X)$ can is shattered by $\Q$ w.r.t. $(\mathcal{X},\sim)$.

($\implies$) By definition VC dimension is the maximal number of points that can be classically shattered by $\Q$. 
So we know that $\op{VC}{\Q} \geq |\mathcal{X} / \sim|$ implies that there exists no deterministic encoder $Z = e(X)$ s.t. for any binary labeling $b$ there is an $f \in Q$ s.t. $f(e(x)) = b(M(X))$.
Then by \cref{lemma:det_sufficient} we know that there exists also no stochastic encoder  $\p{Z|X}$ s.t. $f(Z) = b(M(X))$. 
\end{proof}

\Cref{prop:VC_dimension} gives the requirement of shattering in terms of VC dimension of $\Q$.
We can thus use all the well known results of VC dimensions to to describe minimal sufficient requirements for shatterability.

\begin{manualcor}{\ref{corr:dimension}}[Dimensionality]
Let $\Zc = \mathbb{R}^{d}$. The minimal and sufficient dimensionality $d_{\Q}$ is the smallest $d$ s.t. there exists a discriminative encoder $\p{Z|X} \dP{}$.
$d_{\Q}$ is:
\begin{itemize}
\item is $d_{\Q_l} = |\mathcal{X} / \sim| - 1$ for linear predictors $\Q_l$;
\item is larger for smaller VC dimensions , \ie,  $\op{VC}{\Q^-}  \leq \op{VC}{\Q} \  \implies  d_{\Q^-} \geq d_{\Q}$;
\item increases for any $\Q^- \subseteq \Q$, \ie,  $  d_{\Q^-} \geq d_{\Q}$;
\item decreases with the number of layers $L$ and hidden neurons per layer $H$ for practical MLPs with ReLU activations $\Q_{LH}$, \ie,  $L^+ \geq L$ and $H^+ \geq H$ $\implies d_{\Q_{L^+H^+}} \leq d_{\Q_{LH}}$;
\item is $d_{\U} = 1$ for universal predictors $\U$.
\end{itemize}
\end{manualcor}
\begin{proof}$ $\\
\begin{itemize}
\item The VC dimension $\Q_l$ with domain $\Zc \subseteq \mathbb{R}^d$ is $d +1$ \cite{shalev-shwartz_understanding_2014}. So by \cref{prop:VC_dimension} we have $d + 1 = \op{VC}{\Q_l} \geq |\mathcal{X} / \sim|$ . And thus $d_{\Q_l} = |\mathcal{X} / \sim| - 1$.
\item Increasing the dimensionality of $\Zc$ from $d^-$ to $d > d^-$ can only increase the VC dimension of $\op{VC}{\Q}$ because $\mathbb{R}^{d^-}$ is (isomorphic to) a subspace of $\mathbb{R}^{d}$. So $\op{VC}{\Q^-}  \leq \op{VC}{\Q} \  \implies  d_{\Q^-} \geq d_{\Q}$.
\item If $\Q^- \subseteq \Q$ then clearly $\op{VC}{\Q^-} \leq \op{VC}{\Q}$. 
So by the previous point we have $d_{\Q^-} \geq d_{\Q}$ as desired.
\item Let $\Q_{LW}$ be an MLP with ReLU activation, $W$ parameters (weight and biases), and $L$ layers. In the practical case of $L \ll W^{0.99}$ we have $\op{VC}{\Q} \in \Theta(WL \log(W))$ \cite{bartlett_nearly-tight_2017}.
In particular the VC dimension increases with $L$ and $W$ and so 
$L^+ \geq L$ and $W^+ \geq W$ $\implies d_{\Q_{L^+W^+}} \leq d_{\Q_{LH}}$.
As the number of weights is proportional to the number of hidden units per layer (and the number of layers) we have $d_{\Q_{L^+H^+}} \leq d_{\Q_{LH}}$ as desired.
\item The VC dimension of $\U$ is clearly infinite even with $d_{\U}$. 
In particular, any set of cardinality $|\Xc / \sim|$ (which is finite due to \cref{assmp:finite_rv}) can be shattered because $|\mathbb{R}| > |\Xc / \sim|$.
\end{itemize}
\end{proof}


\Cref{corr:dimension} only discusses the required dimensionality of $\Zc$, but there is also a cardinality requirement.
Indeed, clearly $Z$ has to take enough possible values to be shatterable $\Zc \geq |\Xc / \sim|$.

\begin{proposition}[Marginal support]\label{prop:marginal_supp}
The minimal sufficient cardinality of the marginal support $\supp{\p{Z}}$ is $|\Xc / \sim|$. I.e.:
\begin{itemize}
\item there exists an encoder $\p{Z|X}$ s.t. $\supp{\p{Z}} = |\Xc / \sim|$ and is discriminative $\p{Z|X} \in \dP{}$;
\item there exists no encoder $\p{Z|X}$ s.t. $\supp{\p{Z}} < |\Xc / \sim|$ and is discriminative $\p{Z|X} \in \dP{}$.
\end{itemize}
\end{proposition}
\begin{proof}$ $\\
(Existence) Take the example from \cref{lem:achieve_0} where $Z$ is a maximal invariant and thus has support $|\Xc / \sim|$.

(Non existence) Suppose that there exists a $\p{Z|X}$ s.t. $\supp{\p{Z}} < |\Xc / \sim|$ and can be shattered $\p{Z|X} \in \sP{}$.
Then by \cref{lemma:det_sufficient} there exists a deterministic encoder $e$ with $\Zc < |\Xc / \sim|$ and can be shattered.
Then by \cref{lemma:disc_shatter} $e$ can be shattered.
As $\Zc < |\Xc / \sim|$ there exists two non equivalent examples $x \not \sim x^-$ s.t. $e(x) = e(x^-)$.
Take any binary labeling $b$ that gives a different label for $[x]$ and $[x^-]$. Then by construction $b(M(x)) \neq b(M(x)^-)$ but $e(x) = e(x^-)$ so there exists no $f$ s.t. $f(Z) = f(e(X)) = b(M(X))$ so $Z = e(X)$ cannot be shattered. Contradiction.
\end{proof}

Note that \cref{prop:sample_space} concerns the minimal and sufficient cardinality of the support $\supp{\p{Z}}$, but this directly implies a minimal and sufficient cardinality of the sample space $\Zc$.


\begin{corollary}[Sample space]\label{cor:sample_space}
The minimal sufficient cardinality of the sample space $\Zc$ is $|\Xc / \sim|$
\end{corollary}
\begin{proof}
This directly comes from \cref{prop:marginal_supp} and letting $\Zc = \supp{\p{Z}}$.
\end{proof}

\subsection{Proofs for augmentations}



\begin{manualprop}{\ref{thm:sufficient_refine}}[Refinement and discriminativeness]
Let $\tasksinv{},M,\Q$ be as in \cref{thm:main}. 
Let $\sim_r \subseteq \sim$ be a refinement of the desired equivalence  with maximal invariant $\Mx{r}$.
Let $\oP{\sim}{M} \defeq \argmin_{p(Z|X) \in \sP{}  } \RiskA{M(X)}{\rv Z}$ denote the encoders that can predict $M$ and are shattered w.r.t $(\mathcal{X},\sim)$.
We have:
\begin{equation} \label{eq:sufficient_refine}
\oP{\sim_r}{\Mx{r}} \subseteq \oP{\sim}{\Mx{r}}  \subseteq \oP{\sim}{M}.
\end{equation}
\end{manualprop}
\begin{proof} $ $\\
($\oP{\sim_r}{\Mx{r}} \subseteq \oP{\sim}{\Mx{r}}$)
By \cref{lemma:near_theorem} we know that any $\p{X|X} \in \oP{\sim}{\Mx{r}}$ achieves $\min \RiskA{M(X)}{Z}$.
So we simply need to show that any $\sPr{} \subseteq \sP{}$.
By definition of a refinement and maximal invariant we know that $x \sim_r x^+ \implies  x \sim x^+ \iff M(x) = M(x^+)$, so $M$ is invariant w.r.t $\sim_r$.
By \cref{lemma:invariant} we thus know that there exists an $h$ s.t. $h \circ \Mx{r} = M$.
Now assume that an encoder $p^r(Z|X) \in \oP{\sim}{\Mx{r}}$ and let $b \in 2^{\Mc}$ be any binary labeling.
Then $b(M(X)) = b(h(\Mx{r}(X)))$.
As $b \circ h \in 2^{\Mc^{r}}$ is a binary labeling for the refinement we must have that there exists $\pred{} \in \Q$ s.t. $f(Z) = b(h(\Mx{r}(X)))$ and so $p^r(Z|X) \in \oP{\sim}{M}$ as desired.

($\oP{\sim}{\Mx{r}}  \subseteq \oP{\sim}{M}$)
From \cref{lemma:induction} and the proof of \cref{lemma:near_theorem} we know that  $\sP{} = \oP{\sim}{M}$ so $\oP{\sim}{\Mx{r}}  \subseteq \oP{\sim}{M}$. Note that it is not equal as encoders in $\oP{\sim}{\Mx{r}}$ have the additional constraint of having to be able to predict $\Mx{r}$ which is not implied by shatterability w.r.t. $\sim$.


\end{proof}



% \begin{proposition}\label{prop:finer_harder_optim}
% Let $p(\A|X)$ and $p(\A'|X)$ be sufficient augmenters.
% If the kernel $\sim_{\A}$ of the Bayes predictor for $\A$ is a refinement of $\sim_{\A'}$, then the resulting encoders satisfy
% \begin{equation}
% \argmin_{p(Z|X) \in \sP{}} \RiskA{\A}{Z} \subseteq 
% \argmin_{p(Z|X) \in \sP{}} \RiskA{\A'}{Z}.
% \end{equation}
% %
% \end{proposition}
% \begin{proof}

% \end{proof}


\subsection{Proofs for functional family}

\begin{proposition}\label{prop:smaller_Q_is_better}
Let $\Qm,\Q$ be families s.t. $\Qm \subseteq \Q$. 
Any $p(Z|X)$ satisfying \cref{thm:main} for $\Qm$ also satisfies it for $\Q$.
\end{proposition}
\begin{proof}
\begin{itemize}
    \item by \cref{lemma:disc_shatter} you only need to show that shattering by smaller functional family is shattering by larger
    \item as $\Qm \subset \Q$ if there exists an $f \in \Qm$ s.t. $f(Z) = b(M(X))$ then there also exists an $f' \in \Qm$ by setting $f' = f$.
\end{itemize}
\end{proof}


\subsection{Proofs for generative models}


In \cref{thm:main} we have seen that to have a discriminative encoder one needs to minimize $\RiskA{M(X)}{Z}$, \ie, be able to classify the index of the equivalence class using the right functional family.
There are three issues for optimizing $\RiskA{M(X)}{Z}$ in practice:
\begin{itemize}
\item we do not have access to a maximal invariant $M(X)$, instead, the invariance structure is given by the ability to sample augmented version of the input $A \dsim p(A|X)$ that retain the invariance structure. As we will show in the following one can instead optimize $\RiskA{A}{Z}$.
\item the second issue comes from the fact that $A$ will likely not take value in $\Mc$. As a result minimizing $\RiskA{A}{Z}$ is ill defined because the loss is not defined on the right space. 
Specifically, $\ell : A,f(Z) \mapsto \indeq{A}{\argmax_m f(Z)[m]}$ will never be equal to 1 as $\argmax_m f(Z)[m]$ will give an integer in $[|\Mc|]$ but $A$ can t.v.i. an arbitrary $\Ac$, \eg, image space.
\item the third issue is that accuracy is not smooth, and in practice we would thus prefer minimizing smooth approximations of it to improve optimization.
\end{itemize}

We will now show that we can solve the three issues by instead minimizing the following Bayes risk $\Risk{A}{Z}$ with respect to most practical losses $\ell$.
Specifically, any information preserving loss.

\begin{definition}[Bayes risk for classification]\label{def:bayes_clf}
Let $\ell : \Ac \times \actspace{} \to \mathbb{R}_{\geq 0}$ be an information preserving loss.
Let $\U \defeq \actspace{}^{[|\Mc|]}$ be the unconstrained predictive family from labels $1, \dots,|\Mc|$ to the action space $\actspace{}$.
The Bayes risk from $Z$ to $A$ w.r.t. $\ell,\Q$ for classification, denoted $\RiskL{A}{Z}{\mathrm{clf},\ell}$, is the Bayes risk when first performing classification and then considering the unconstrained Bayes risk from the predicted class to $A$. I.e. 
\begin{equation}
\RiskL{A}{Z}{\mathrm{clf},\ell} \defeq \inf_{g \in \U} \inf_{f \in \Q} \Ep{\p{A|X}\p{Z|X}}{\ell(A, g(\argmax_m f(Z)[m] )}
\end{equation}
As all Bayes risk w.r.t. $\ell$ are for classification we will simply denote it $\Risk{A}{Z}$.
\end{definition}

It turns out that minimizing the Bayes risk for classification \cref{def:bayes_clf} is equivalent to predicting $M(X)$ when the augmentations $A$ retain the same equivalence structure. 

\begin{proposition}[Using augmentations and losses]\label{prop:using_aug_loss}
Let $\ell$ be any information preserving loss.
Let $\p{A|X}$ be any augmentor s.t. any Bayes predictor $\bayes{A|X}$ is a maximal invariant, \ie, $x \sim x^+ \iff \bayes{A|X}(x) = \bayes{A|X}(x^+)$.
Then:
\begin{equation}
\argmin_{\p{Z|X} \in \sP{}} \RiskA{M(X)}{Z} = \argmin_{\p{Z|X} \in \sP{}} \RiskL{A}{Z}{\mathrm{clf},\ell}  
\end{equation}
\end{proposition}
\begin{proof}$ $\\
First we will show that $\min_{\p{Z|X}} \RiskL{A}{Z}{\mathrm{clf},\ell} =  \Risk{A}{X}$.
Then that an encoder $\p{Z^*|X}$ achieves that risk if and only if $\exists f \in Q$ s.t. $M(X) = \argmax_m f(Z^*)[m]$, which is equivalent to $\p{Z^*|X} \in \argmin_{\p{Z|X}} \RiskA{M(X)}{Z}$.
Finally we note that due to \cref{lemma:achieve_0,lemma:disc_shatter} we have $\argmin_{\p{Z|X}} \RiskA{M(X)}{Z}  = \argmin_{\p{Z|X} \in \dP{}} \RiskA{M(X)}{Z} = \argmin_{\p{Z|X} \in \sP{}} \RiskA{M(X)}{Z}$ and so proving the unconstrained $\argmin_{\p{Z|X}} \RiskA{M(X)}{Z} = \argmin_{\p{Z|X}} \RiskL{A}{Z}{\mathrm{clf},\ell} $ is sufficient.

%Second note that $\p{Z^*|X} \in \argmin_{\p{Z|X}} \RiskL{A}{Z}{\mathrm{clf},\ell}$ if and only if there exists a function $\phi$ s.t. $\phi(Z^*)= M(X)$.,

Let $Z^*$ be the one hot encoding of $M(X)$ as in \cref{lemma:achieve_0} then by letting $f$ be the identity function we have
\begin{align}
\RiskL{A}{Z^*}{\mathrm{clf},\ell} 
&\defeq \inf_{g \in \U} \inf_{f \in \Q} \Ep{\p{A|X}\p{Z|X}}{\ell(A, g(\argmax_m f(Z)[m] )} \label{eq:g_arg_f} \\
&\geq \inf_{g \in \U} \Ep{\p{A|X}\p{Z|X}}{\ell(A, g(M(X))}  & \text{Identity} \\
%&\defeq \RiskQ{A}{M(X)}{\U} \\
&\geq  \Ep{\p{A|X}\p{Z|X}}{\ell(A, \bayes{A|X}(X)}  & \text{\cref{lemma:max_invariant}} \\
&\defeq \RiskQ{A}{X}{\U}
\end{align}
Where we fixed $f$ to be the identity (possible by \cref{assmp:binary_linear}).
We also let $g$ be the function from $M(X)$ to $\bayes{A|X}$ which exists as $\U$ is unconstrained and $\bayes{A|X}$ is a maximal invariant by assumption so there exists a bijection $b$ s.t. $\bayes{A|X} = b(M(X))$.
We thus have $\RiskL{A}{Z^*}{\mathrm{clf},\ell} \geq \Risk{A}{M(X)} \geq \Risk{A}{X}$.
Note that by the risk DPI (\cref{lemma:dpi}) we also have $\RiskL{A}{Z^*}{\mathrm{clf},\ell} \leq \Risk{A}{X}$ from which we conclude $\min_{\p{Z|X}} \RiskL{A}{Z}{\mathrm{clf},\ell} =  \Risk{A}{X}$.

In \cref{eq:g_arg_f} we see that the function mapping $Z$ to $\actspace{}$is a composition between the argmax predictor $\Tilde{f} : Z \to [|\Mc|]$ and the unconstrained $g : [|\Mc|] \to \actspace{}$.
As $\min_{\p{Z|X}} \RiskL{A}{Z}{\mathrm{clf},\ell} = \Risk{A}{X}$ we have that $\Tilde{f} \circ g$ must be equal to a maximal invariant as it must be a equal to a Bayes predictor which by assumption is a maximal invariant.
As $g$'s domain has cardinality $|\Xc / \sim|$ and its image is a maximal invariant, it must be a bijection so by \cref{lemma:max_invariant} $\Tilde{f}$ must also be a maximal invariant.
From which we conclude that $\exists f \in Q$ s.t. $M(X) = \argmax_m f(Z)[m]$.

Now let us show that that $\p{Z^*|X} \in \argmin_{\p{Z|X}} \RiskA{M(X)}{Z}$ if and only if there exists a function $f \in Q$ s.t. $\argmax_m f(Z^*)[m] = M(X)$.
Indeed $\min_{\p{Z|X}} \RiskA{M(X)}{Z} \geq \RiskA{M(X)}{X} = 0$ because $Z=X$ is a valid representation, so we have $\RiskA{M(X)}{Z^*} = 0$ which is achieved if and only if $\exists f \in Q$ s.t. $M(X) = \argmax_m f(Z^*)[m]$ as desired.
\end{proof}

\Cref{prop:using_aug_loss} is very nice as it says that we do not need access to the maximal invariant as long as we have access to the right augmentation.
For example in the case of generative model, it is typical to use the mean squared error, in which case the Bayes predictor is the conditional expectation $\Ep{A}{X}$, the requirement is thus to have $\Ep{A}{X} = \Ep{A}{M(X)}$. 
This will rarely be the case in practice for standard augmentations but by \cref{prop:sufficient_refine} we know that $x \sim x^+ \implies \bayes{A|X}(x) = \bayes{A|X}(x^+)$ is also sufficient, which typically holds in practice. 
E.g. for MNIST it says that the expected (over augmentation) digit should essentially not be another digit.


\subsection{Proofs for contrastive models}

\subsection{Proofs for self-distillation }


\clearpage
\newpage

==> appendices/proofs/discriminative.tex <==

% Intuitively, the proof of the main theorem goes as follows:
% \begin{enumerate}
%     \item There exists
%     \item \dots
% \end{enumerate}

\ydnote{should add a few bullet points to give the intuition of the proof of main theorem}

First let us show that we can achieve the minimal worst case risk, and let us provide an example of optimal representation.

\begin{lemma}[Perfect worst risk]\label{lemma:achieve_0}
For any $\Q$ that is at least linear with binary weights (\cref{assmp:binary_linear}) there exists an encoder $\p{Z^* | X}$ that achieves the unconstrained worst excess Bayes risk on all $(\Xc,\sim)$-invariant tasks, \ie,
%, \ie, for all $Y \in \tasksinv{}$ we have
\begin{equation}
%\Risk{Y}{Z} = \RiskQ{Y}{Z}{\U}
\min_{\p{Z|X}} \dists{} = 0
\end{equation}
\end{lemma}
\begin{proof}
This can easily be seen by taking $Z^*$ to be a one hot representation of the equivalence class and $\pred{} \in \Q$ be the necessary aggregation function represented as linear equation with binary weights.

Specifically, let $Z^* = \onehot{\nequiv}{M(X)}$ where $M$ is a maximal invariant that maps inputs to an index of the equivalence classes.
Such representation exists by \cref{assmp:rep_space}.


As $\mathbf{e}_i$ is a bijection we have that $Z^*$ is a maximal invariant for $\sim$ by \cref{lemma:max_invariant} because it is a composition between a bijection and a maximal invariant.
By \cref{def:inv_task}, we have that for any $Y \in \tasksinv{}$ the Bayes predictor $\Bpred{}$ is invariant w.r.t. $(\Xc,\sim)$.
As $Z^*$ is a maximal invariant and $\Bpred{}$ is invariant, by \cref{lemma:invariant} there must exist a function $h$ s.t. $h(Z^*) = \Bpred{}(X)$.
\ydnote{need to change to a bayes predictor now (because not all are invariant)}
As the codomain of the Bayes predictor $\Bpred{}$ is also a one hot encoding, we have that $h$ is a function between one hot encodings and can thus be represented by a linear function with binary weights, \ie, $h(Z^*) = W^T Z^*$ where $W \in \set{0,1}^{|\Mc| \times |\Yc|}$ serves as an OR gate.
As $h$ is linear with binary weights it is by \cref{assmp:binary_linear} in $\Q$.
Putting all together we have that for any $Y \in \tasksinv{}$ there exists an $h \in \Q$ so that $\Risk{Y}{Z} \leq \RiskQ{Y}{Z^*}{\set{h}} = \RiskQ{Y}{X}{\set{\Bpred{}}} = \RiskQ{Y}{X}{\U}$.
We conclude the proof by noting that for any $Z$ we have $\Risk{Y}{Z} \geq \RiskQ{Y}{Z}{\U} \geq \RiskQ{Y}{X}{\U}$ where the last inequality comes from the DPI of Bayes risk \cref{lemma:dpi}.
We thus have $\Risk{Y}{Z} = \RiskQ{Y}{X}{\U}$ and so $\dists{} = 0$.
\end{proof}

One important implication of \cref{lemma:achieve_0} is that the set of encoders that are discriminative for the worst-case excess risk is the same as the set of encoders that are discriminative for the average case.
In other words we could replace the supremum in \cref{def:discriminative} by any expectation with support over all invariant tasks, and that would not change any of the theory.

Now we will show that under \cref{assmp:closed}, the binary $\sim$-shatterability from \cref{def:shatter} 
implies $k$-ary shatterability.
The main idea intuition is that we can always achieve predict a desired $k$-ary invariant labelling by combining (due to \cref{assmp:closed}) a ${(k-1)}$-ary predictor with the binary predictor that distinguishes the wrong predictions from the rest.

As previously stated, one can drop \cref{assmp:closed} by changing the binary shatterability requirement to a $k$-ary shatterability (instead of probing it from assumptions).

\begin{lemma}[Binary shatterability implies $k$-ary shatterability]\label{lemma:kary_shatterability}
Let $\Q$ satisfy \cref{assmp:closed}.
If an encoder $\p{Z |X}$ is binary  $(\Xc,\sim)$-shattered by $\Q$ then it is $k$-ary $(\Xc,\sim)$-shattered by $\Q$.
\end{lemma}
\begin{proof}
We will prove the statement by induction, \ie, we suppose that for any $1 < i < k$ we have that $i$-ary shatterability holds and want to prove that it implies $k$-ary shatterability.


We will prove the induction by contradiction. 
Suppose that $k$-ary shatterability does not hold.
Then by definition there exists a $k$-ary invariant labelling $\labelingk{k}$ s.t. no $f_{\scriptscriptstyle k} \in Q$ satisfies $\prediction(f_{\scriptscriptstyle k}(Z)) \aseq \labelingk{k}(X)$. 
Construct $\labelingk{k-1}$ by merging the two last classes, \ie, $\labelingk{k-1}(x) = \labelingk{k}(x)$ if $\labelingk{k}(x) < k $ and $\labelingk{k-1}(x) = k - 1$ otherwise.
By construction $\labelingk{k-1}$ is a ${(k-1)}$-ary invariant labelling so by the induction assumption there exists an $f_{\scriptscriptstyle k-1} \in \Q$ s.t. $\prediction(f_{\scriptscriptstyle k-1}(Z)) \aseq \labelingk{k-1}(X)$.
Now let $\labelingk{2},\labelingk{2}'$ be functions that indicates whether the unpredictable labelling is equal to the last class $\labelingk{2} : x \mapsto \indeq{\labelingk{k}(x)}{k}$ and similarly $\labelingk{2}' : x \mapsto \indneq{\labelingk{k}(x)}{k}$.
By construction $\labelingk{2},\labelingk{2}'$ are binary invariant labelling, so again by the induction assumption there exists an $f_{\scriptscriptstyle 2},f_{\scriptscriptstyle 2}' \in \Q$ s.t. $\prediction(f_{\scriptscriptstyle 2}(Z)) \aseq \labelingk{2}(X)$ and $\prediction(f_{\scriptscriptstyle 2}'(Z)) \aseq \labelingk{2}'(X)$.

By \cref{assmp:closed} we can then use $f_{\scriptscriptstyle k-1},f_{\scriptscriptstyle 2},f_{\scriptscriptstyle 2}'$ to construct the desired an $f_{\scriptscriptstyle k} \in Q$ satisfying $\prediction(f_{\scriptscriptstyle k}(Z)) \aseq \labelingk{k}(X)$.
Specifically, we can construct the function mapping to the logits of class $k-1$ by $f_{\scriptscriptstyle k}^{k-1} = f_{\scriptscriptstyle k-1}(\cdot)[k-1] + f_{\scriptscriptstyle 2}'$, the function mapping to the logits of class $k$ by $f_{\scriptscriptstyle k}^{k} = f_{\scriptscriptstyle k-1}(\cdot)[k-1] + f_{\scriptscriptstyle 2}$ and then concatenate all the logits to get the desired $f_{\scriptscriptstyle k} = \cat{f_{\scriptscriptstyle k-1}(\cdot)[\slice{}k-2]}{f_{\scriptscriptstyle k}^{k-1},f_{\scriptscriptstyle k}^{k}}$.
Indeed, by construction the first $k-2$ classes were already dealt with correctly, and we simply used $f_{\scriptscriptstyle 2}$ and $f_{\scriptscriptstyle 2}'$ a positive component to the right class (we used two functions $f_{\scriptscriptstyle 2},f_{\scriptscriptstyle 2}'$ to deal with zero values logits) and distinguish examples form class $k$ and $k-1$.
The resulting function thus satisfies $\prediction(f_{\scriptscriptstyle k}(Z)) \aseq \labelingk{k}(X)$ which leads to a contradiction.
We thus have that $k$-ary shatterability, which concludes the proof due to induction (the base case being binary).
\end{proof}


% \begin{lemma}[Induction]\label{lemma:induction}
% Let $\Q$ a predictive family satisfying \cref{assmp:binary_linear}.
% If for any $(\Xc,\sim)$-invariant binary labeling $b \in  \set{0,1}^{\Xc}$ there exists an $\pred{} \in \Q$ s.t. $\pred{}(Z) = b(X)$ then for any $(\Xc,\sim)$-invariant $k$-labelling $L \in  \set{1, \dots, k}^{\Xc}$ there exists an $\pred{}' \in \Q$ s.t. $\pred'(Z) = L(X)$.
% \end{lemma}
% \begin{proof}
% \begin{itemize}
% \item use proof by induction to show that if you can predict any invariant $n$-labeling and any binary labeling then you can perform any $(n+1)$-labelling
% \item for any invariant $(n+1)$-labelling $L^+$ you can merge two labels to get an invariant $n$-labelling $L$, which is predictable by assumption of the induction.
% \item now take one of the two labels you merged and perform a one-vs-rest task which is invariant binary labeling
% \item as $\Q$ is closed under compostion of linear functions with binary weight matrices you can sum the result of both preditive tasks
% \item after some algebra easy to show that this will perfectly predict the desired $(n+1)$-labelling.
% \end{itemize}
% \end{proof}

Putting all together let us prove the minimal and sufficient requirement for discriminativeness.




\begin{manualthm}{\ref{thm:main}}[Minimal sufficient requirements for discriminativeness]
Let $M(X)$ be any maximal invariant \wrt{} $(\Xc,\sim)$, and $\tasksinv{}$ be all invariant tasks \wrt{} $(\Xc,\sim)$.
An encoder $\p{Z|X}$ is discriminative for $\tasksinv{},\Q$ if and only if it minimizes the $\Q$-predictability of the maximal invariant while being $(\Xc,\sim)$-shattered by $\Q$, \ie, 
\begin{equation}\label{appx:eq:thm}
\p{Z|X} \in \dP{} \iff \p{Z|X} \in \argmin_{\p{Z|X} \in \sP{}} \Risk{M(X)}{Z}
\end{equation}
\end{manualthm}
\begin{proof}
We will first prove necessity, which comes from the fact that $M(X)$ and binary labeling are in $\tasksinv{}$.
We then prove sufficiency which comes from the fact that by \cref{lemma:kary_shatterability} any invariant labeling can be predicted under shatterability, including predicting all the Bayes predictions.


$(\implies)$ By \cref{lemma:achieve_0}, all discriminative encoders achieve $\Risk{Y}{Z} = \RiskQ{Y}{X}{\U}$ for all $Y \in \tasksinv{}$.
By \cref{def:shatter} any binary invariant labeling $\labelingk{2}$ is an invariant task  $\labelingk{2}(X) \in \tasksinv{}$ as the Bayes predictor $\prediction(\Bpred)=\labelingk{2}$ is invariant.
As $\labelingk{2}(X)$ is a deterministic labeling we have $\Risk{\labelingk{2}(X)}{Z} = \RiskQ{\labelingk{2}(X)}{X}{\U} = 0$. By the definition and non-negativity of the \acc{} loss, there must exist an $f \in \Q$ s.t. $\prediction(f(Z)) \aseq{} \labeling{}(X)$.
As this is true for binary labeling, we have that discriminativeness implies shatterability.
By the same argument we have that maximal invariants are a deterministic invariant task  $M(X) \in \tasksinv{}$, so $\Risk{M(X)}{Z} = \RiskQ{M(X)}{X}{\U} = 0$.
Discriminativness thus implies perfect predictability of maximal invariants, which can be rewritten as a constrained optimizatin problem. 
Indeed, the constrain does not impact the predictability of the maximal invaraint due to the existence of a perfect encoder (\cref{lemma:achieve_0}).
This concludes the necessity proof.

$(\impliedby)$  Suppose that $\p{Z|X}$ is a minimizer of the r.h.s. of \cref{appx:eq:thm}.
By \label{def:inv_task} for any $Y \in \tasksinv{}$ there exists an invariant Bayes predictor $\Bpred$.
As it is an invariant (deterministic) function of $X$, we have that $\prediction(\Bpred(\cdot))$  is also an invariant determinsitic function of $X$ (it is easy to show that it is $\prediction(\Bpred(\cdot)) = \argmax_{y \in \Yc} p(y|x)$ were the same element $y$ is selected for all equivalent $x$). $\prediction(\Bpred(\cdot))$ is thus an invariant labeling $\labelingk{|\Yc|}$.
By \cref{lemma:kary_shatterability},  binary shatterability of $\p{Z | X}$ thus implies that there exists an $f \in \Q$ s.t. $\prediction(f(Z)) \aseq{} \prediction(\Bpred(X))$.
For all invariant tasks we thus have $\Risk{M(X)}{Z} = \RiskQ{M(X)}{X}{\U} = 0$ so $\p{Z|X} \in \dP{} $ as desired. 
\end{proof}

As seen in the proof, binary shatterability implies discriminativeness. 
We neverthless put emphasize the maximal invariant in \cref{appx:eqn:task_invariance}, because predictability of the maximinal invariant is more computationally efficient and, as shown in \toappx{}, implies discriminativeness with high likelihood when the dimension is large enough.




==> appendices/results_old.tex <==
\subsection{Approximations}

In this section we evaluate the effect of different approximations that we had to do for computational reasons.

\subsubsection{Effect of number of subtasks}

In \tocref{} we looked at the worst possible performance on \tofill{} randomly sampled binary tasks. This is an approximation of the real metric that we care (see \tocref{}), \ie, which is the worst possible invariant task.
The number of subpartitions, i.e., deterministic tasks to consider, is given by the Bell number $B_n$ \tocite{}. Solving that many tasks to find the the worst possible is computationally prohibitive. For example when $|\mathcal{M}|=10$ as is the case for MNIST, that would require taking the max over $B_n=115975$.
We thus make two assumptions:
\begin{itemize}
\item consider only binary tasks, as those are the ones that aggregate the most, and we conjecture that if we can solve all binary subpartions then we can solve all k-ary partitions; 
\item sample a few tasks, as considering all binary tasks for MNIST would require $S(|\mathcal{M}|,2)=511$ tasks which is still prohibitive. Here $S$ is the Stirling number of the second kind.
\end{itemize}
We now evaluate those approximations for MNIST. 
We do so for generative and contrastive ISSL models, both for standard and our variants.

\input{figures/mnist/effect_n_tasks}

\paragraph{The number of tasks has less effect on our ISSL.}
 \cref{fig:effect_n_tasks} shows that the number of tasks (number and type) has less on our ISSL (first two columns) compared to standard ISSL (last two columns).
Indeed, the performance gap between our ISSL and standard ISSL increases as the number of considered tasks increases from $4 \to 64$.
For contrastive ISSL: $0.3 \to 0.55$ pp.
For generative ISSL: $13 \to 17$ pp.
This suggests that using more tasks would only make our ISSL seem more compelling, and thus using fewer tasks due to computational reasons does not change the main take aways.

\paragraph{Binary tasks are better approximations.}
We see on  \cref{fig:effect_n_tasks}, as hypothesized, the hardest tasks seem to be binary tasks. Note that this is not the case for all binary tasks, which is why for standard generative model, binary tasks are have higher performance than ``all tasks''. For average case, it makes sense that binary tasks are easier simply because random prediction is already much better ($50\%$ against $10\%$ for all tasks).
This supports our choice of binary tasks throughout our paper.


\paragraph{32 tasks gives a good approximation.}
From  \cref{fig:effect_n_tasks}, we see that the accuracy decreases significantly and monotonically with the number of tasks.
Although more tasks continue decreasing the accuracy, $32$ generally seems to give decent approximations while being manageable computationally. This is why we use 32 tasks whenever we want good approximations of the worst case performance.
Otherwise we use 16 tasks throughout the paper.


\clearpage
\newpage

\subsection{Testing the theory}
\label{appx:results:testing_theory}

\subsubsection{Controlled experiments}
\label{appx:results:controlled}

In the main paper we have evaluated the theory in well controlled experiments.
Here we provide all the results that have only been hinted towards in the main text due to space limitation.


\input{figures/controlled/regularization}

\paragraph{Effect of regularization on dimensionality and sample efficiency?}
As discussed in the main text, the minimal achievable dimensionality and sample efficiency can only be achieved if equivalent examples $x \sim x^+$ get mapped to the same representations $z$, but the ISSL objective only ensures that non-equivalent examples $x \not\sim x^-$  are mapped to different representations $z,z^-$.
To achieve the former we can add an additional regularizer (see \tocref{}).
 \Cref{fig:regularizers} shows indeed that adding a regularizer is necessary to achieve the optimal dimension $d(\Q)=10$ (\cref{fig:reg_dim}) and sample efficiency $\rS{}$ (\cref{fig:reg_samples}).
Furthermore, we see that in both cases the need for a regularizer decreases when training for longer.
This suggests that training for longer can have the desired implicit regularization effect, which could explain why long training times are so important in practical ISSL \cite{}.
We hypothesize that the implicit regularzation effect comes from the noise in SGD which essentially minimizes some form of $\MI{Z}{X}$ \cite{shwar}. %Opening black box


\input{tables/controlled/appcs/exact_losses}
\input{tables/controlled/appcs/exact_losses_test}
\paragraph{Effect of using the wrong loss?}
In \tocref{} we prove that any \tofill{} loss can be used during ISSL to achieve optimal representations, and surprisingly this is independent of the choice of downstream losses.
\Cref{tab:exact_losses} empirically supports our claim by showing that any of MSE / hinge / log loss used during ISSL can learn optimal representations.
Furthermore, we see that performance w.r.t. specific downstream loss (MSE / hinge / 0-1/ log loss) is uncorrelated with the loss used during ISSL.
Note that our theoretical results say nothing about when ISSL is not perfect (e.g. approximate optimizers and only access to samples) in which case the choice of loss is actually important.
\Cref{tab:exact_losses_test} shows that even when ISSL is not optimal (using access to samples) the choice of loss for ISSL and prediction still seem uncorrelated.



\input{tables/controlled/appcs/exact_permMx}

\paragraph{Do augmentations need to retain labels?}
It is often said \tocite{} that data augmentations should not change the label of the underlying example. 
We have seen in \tocref{} that actually this is not a necessary requirement, the necessary and sufficient requirement essentially says that if the Bayes predictor of the augmentation is the same then so should the labels the examples, i.e., $\bayesA{\A \cond X}(x) = \bayesA{\A \cond X}(x')  \implies x \sim x'$.
In practice this means that input examples (e.g. an image of an ``8'') can be augmented to output examples that would generally have different labels (e.g. an image of a ``9''), as long as this is the case for all equivalent examples (e.g. all ``8'' get augmented to ``9'').
We show that this indeed the case in \cref{tab:exact_permMX} by comparing exact augmentations to augmentations to permuted $M(X)$ in the case of exact (``train'') and samples estimates (``test'') ISSL.
When using exact ISSL, this should be quite intuitive as this simply corresponds to permuting the weight matrix of the last linear predictor.
Perhaps more suprisingly we show in \cref{tab:cntr_permMX} that the same holds when using contrastive learning and finite samples, which disproves the typical explanation of contrastive learning as ``bringing augmented and non-augmented examples closer together''.


\subsubsection{Practical setting}
\label{appx:results:practical}

In the following we show that the trends we saw in the main controlled experiments (\cref{sec:controlled_exp}) in the typical practical setting where we use approximate ISSL objectives (here contrastive) and do not assume access to the underlying unlabelled distribution $p(X)$.
Although our theory does not cover this setting we show that generally the same trend hold, which suggests that our theory provides the right intuition in practical settings and can likely be generalized to cover those such case of practical/approximate ISSL.
To minimize computation we run only the core experiments.


\input{figures/cntr_controlled/aug}

\paragraph{Effect of augmentations on required dimensionality?}
In \cref{fig:aug_dim} we have seen that, as predicted by theory,  using any sufficient augmentation one can achieve perfect performance for a certain dimensionality of $Z$.
Importantly, this required dimensionality decreases as the augmentation becomes coarser.
\Cref{fig:cntr_aug_dim} shows exactly the same trend with best performance achieved from a dimensionality of $d(\Q)=10$ when using optimal augmentations.


\paragraph{Effect of augmentations on sample efficiency?}
In \cref{fig:aug_sample} we have seen that, as predicted by theory, using any sufficient augmentation one can achieve perfect performance when downstream predictors are trained on enough samples.
Importantly, this required number of samples decreases as the augmentation becomes coarser.
\Cref{fig:cntr_aug_sample} shows exactly the same trend with best performance achieved from a dimensionality of $\op{S_{\scriptscriptstyle \Q^-}}{\tasksinv{}|Z}=10$ when using optimal augmentations.



\input{figures/cntr_controlled/func_family}

\paragraph{Effect of using the wrong $\Q$?}
\tofill{}
\ydnote{
This is the only currently bad results, not sure what do here}



\paragraph{Effect of $\Q$ on the dimensionality?}
In \cref{fig:V_dim} we have seen that, as predicted by theory, more complex (in terms of VC dimension) downstream predictors require a smaller dimensionality of $Z$ to achieve the highest possible predictions.
\Cref{fig:V_dim} shows that the same trends holds for for approximate contrastive learning.
Just as the theory says, the optimal prediction seems to be achieved when the VC dimension is $|\mathcal{X} / \sim|-1$ which for linear predictor is $9$.



\input{tables/controlled/appcs/cntr_permMx}

\paragraph{Augmentations do not need to retain labels}
In \cref{tab:exact_permMX} we have seen that, as predicted by theory, the augmentation can change the underlying labels as long as the change is predictable.
\cref{tab:cntr_permMX} shows the same essentially holds when considering the practical setting of contrastive (i.e. approximate) ISSL and evaluating on unseen test points.





\subsubsection{Approximate ISSL objectives: generative, contrastive, self-distillation}
\label{appx:results:approx_ISSL}

In the last two subsection we have shown experiment that support our theory in
\begin{inlinelist}
\item settings that are as close as possible to our assumptions, i.e., exact ISSL with $p(X)$;
\item practical settings with contrastive learning and finite sample estimation.
\end{inlinelist}
In the following we show that the same trend essentially hold for other approximate ISSL, specifically, generative and self-distillation models.
As all experiment require hundreds of runs, we consider focus on the small MNIST dataset which is sufficient to show that the same trends hold and avoids unnecessary computation.
%Importantly, this is only about the approximate ISSL object, but we still focus on the the case where the unlabelled distribution $p(X)$ is accessible, we consider finite sample setting in the next section.

% All results are summarized in \cref{tab:appcs:mnist}.
% The first row ``supervised'' shows the performance of a supervised model, while the next four blocks ``exact'', ``generative'', ``contrastive'', ``self-distillation'' refer to the objective used of ISSL (see \tocref{}).
% In each block ``Standard'' corresponds to the standard objective for that type while ``ours'' refer to our proposed small modifications.
% All rows use standard augmentations besides the ``opt. aug.'' rows which use optimal augmentations.
% ``$\Q$'' and ``$\Q^+$'' refer to the predictive family of both the predictor and ISSL.
% By default no regularization is used besides in the rows ``reg.''.
% For columns $\rS{}$ is the estimated sample efficiency, $d(\Q)$ is the estimated minimal required dimension, 
% ``$\RiskA{M(X)}{Z}$  train'' shows the training performance, \ie, says whether the information is decodable and assumes the unlabeled $p(X)$ is seen during training. 
% ``$\RiskA{M(X)}{Z}$'' is the same but on the test set, \ie, the practical objective people care about.
% ``$\sup_Y \RiskA{Y}{Z}$'' shows the test performance on the worst invariant task, \ie, coarsening of the MNIST task such as whether the digit is odd or even.
% ``100 labels'' shows the test performance $\RiskA{M(X)}{Z}$ but when only a few labels are seen ,\ie, essentially semi-supervised learning.
% ``$\times$'' means that we did not find a good estimate of the desired values.

% \input{tables/controlled/appcs/mnist}

% \ydnote{might just drop all the columns besides d and s estimate. I'm not sure what the rest gives as information.
% Might even just keep them for opt aug and non opt aug.
% }



\input{tables/controlled/appcs/mnist_samples}



\paragraph{Does approximating the ISSL objective change the required sample efficiency $\rS{}$?}
From \tocref{} we know that the required sample efficiency should be $\rS{}=10$ when using optimal augmentations.
We have seen in \cref{fig:aug_sample} and \cref{fig:cntr_aug_sample} that this value is recovered both in the controlled (exact ISSL) and practical (contrastive) setting for CIFAR10.
\Cref{tab:appcs:mnist} shows that the same $\rS{}=10$ essentially holds for MNIST and self-distillation and generative approximations of the ISSL objective.
Note that for self-distillation we actually get $\rS{}=100$, we believe that this is due to practical optimization issues.
Importantly when using non standard augmentations we get larger $\rS{}$ as suggested in \cref{fig:aug_sample}.


\input{tables/controlled/appcs/mnist_dim}

\paragraph{Does approximating the ISSL objective change the required dimensionality $d(\Q)$?}
From \tocref{} we know that the required dimensionality should be $d(\Q)=9$ when using optimal augmentations.
\ydnote{actually it's annoying because in reality the required dimensionality should be 9 but we only tested the closest 9}
We have seen in \cref{fig:aug_dim} and \cref{fig:cntr_aug_dim} that this value is recovered both in the controlled (exact ISSL) and practical (contrastive) setting for CIFAR10.
\Cref{tab:appcs:mnist} shows that the same $d(\Q)=10$ essentially holds for MNIST and self-distillation and generative approximations of the ISSL objective.
Note that for self-distillation we actually get $d(\Q)=16$ which is the next dimension we tested, we believe that this is due to practical optimization issues.
Importantly when using non standard augmentations we get larger $d(\Q)$ as suggested in \cref{fig:aug_dim}.


\input{tables/controlled/appcs/mnist}



\clearpage
\newpage

\subsection{Realistic}
\label{appx:results:realistic}

\input{tables/realistic/appcs}

==> appendices/testing_theory.tex <==

\subsection{Controlled experiment}
\label{sec:controlled_exp}

We tested our theory in a  controlled setting as close as possible to our theory.
Specifically, unless stated otherwise, we used
\begin{inlinelist}
\item exact ISSL \cref{eq:obj_to_appx} to avoid approximate objectives;
\item the maximal invariant $\Mx{A}$ given by the true labels $Y$ (CIFAR10; \cite{krizhevsky_learning_2009}) which simulates knowledge of the tasks' equivalence structure;
\item the worst accuracy over 10 coarsenings of the CIFAR10 task $\tasksinv{}$ to approximate $\distsA{}$ in \cref{eq:worst_case},
\item the test distribution during ISSL to simulate access to infinite unlabeled data $p(X)$;
\item a regularizer enforcing the encoders invariance as in \cref{prop:sample_eff_support} by minimizing $\| Z_\theta(x) - Z_\theta(x^+) \|$. 
\end{inlinelist}
In \cref{sec:appx:res:testing_theory} we show similar results in the more natural settings of CISSL trained with standard augmentations and no access to $p(X)$.
All results are over 3 seeds.

\ydnote{
figure comments:
Had to drop y axis for space reasons for \cref{fig:augmentations} (it's the same as \cref{fig:aug_sample})

todo: Need to increase fonts and lines in \cref{fig:predictors}.
}


\input{figures/controlled/controlled}

First, we considered the effect of predictors $\Q$ on ISSL. 
We used three families $\Q^- \subseteq \Q \subseteq \Q^+$:
a linear $\Q^-$, a small MLP $\Q$ (hidden unit: $[10]$), and a large MLP $\Q^+$ (hidden units: $[2048,2048]$).


\paragraphQ{Effect of $\Q$ on dimensionality}
\Cref{cor:dimension} says that the required dimensionality $d_{\Q}$ is the VC dimension of $\Q$.
To test that we swept over dimensionality of $Z$ and predictor size.
As predicted, 
\cref{fig:V_dim} shows that for linear $\Q^-$ the required dimensionality is $d_{\Q^-}=|\mathcal{X} / \sim|-1 = 9$, while it shrinks for more complex predictors: $d_{\Q}\approx5$, $d_{\Q^+}\approx2$.




\paragraphQ{Effect of using the wrong $\Q$}
\Cref{prop:predictive_family} shows that one has to perform ISSL with respect to a family $\Qissl$ that is (at most) a subset of the true downstream predictors $\Qpred$.
We tested this by sweeping predictor size for $\Qissl$ and $\Qpred$. 
As predicted, \cref{fig:V_heat} shows perfect performance only when $\Qissl \subseteq \Qpred$.
This suggests that it is important to consider downstream $\Qpred$ during ISSL.

We then considered augmentations or equivalences $\sima$ used for ISSL. % while keeping the downstream tasks equivalence fixed to the one given CIFAR10 labels.
Specifically: 
(``Exact'') 10 classes given by CIFAR10 labels; 
(``Finer'') 100 classes given by aggregating $10\%$ of same-label images; 
(``Std'') standard data augmentations;
(``None'') no augmentations;
(``Coarser'') 2 classes given by aggregating labels;
(``Rand'') 1000 classes given by aggregating any images.


\paragraphQ{Effect of augmentations on dimensionality}
As predicted in \cref{sec:augmentation}, \cref{fig:aug_dim} suggests that ISSL with finer equivalences (``Finer'' / ``Std'' / ``None'') than desired (``Exact'') achieve optimal performance on invariant tasks but require higher dimension $Z$.
In contrast other augmentations  (``Coarser'' / ``Rand'')  underperform.
By construction ``Exact'' and ``Finer'' have 10 and 100 equivalence classes, and we see that the required dimensionality $d(\Q^-)$ is 9 and 99 as predicted by  \cref{cor:dimension}.



\paragraphQ{Effect of augmentations on sample efficiency}
As predicted in \cref{sec:augmentation}, \cref{fig:aug_sample}
shows that augmentation that give finer equivalences (``Finer'' / ``Std'' / ``None'') than desired (``Exact'')  achieve optimal performance but require more downstream samples.
Furthermore, for ``Exact'' and ``Finer'' the required sample size is the number of classes 10 and 100 as predicted by \cref{prop:sample_eff_support}.


% \paragraphQ{Effect of regularization}
% \Cref{prop:sample_eff_support} shows that the minimal required sample size $\rS{} = \nequiv{}$ is achieved if the encoder is invariant. 
% \Cref{fig:aug_sample} shows that any downstream task $Y \in \tasksinv{}$ can indeed be performed using only  $\rS{} = 10$ samples.
% We performed the same experiment without regularizing $\| Z_\theta(x) - Z_\theta(x^+) \|$ and found $\rS{} = 64$.
% This shows that discriminative encoders can have different sample efficiency and invariance achieves the minima.
% Details at \cref{sec:appx:res:testing_theory}.

==> figures/cntr_controlled/func_family.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[t]{0.33\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cntr_controlled/cntr_V_heatmap_smallZ_final_min.pdf}
         \caption{$\Qissl$ vs $\Qpred$}
         \label{fig:cntr_heat}
     \end{subfigure}
     %\hfill{}
     \qquad\qquad
     \begin{subfigure}[t]{0.3\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cntr_controlled/cntr_V_lines_acc_vs_dim.pdf}
         \caption{Effect of $\Q$ on dim.}
         \label{fig:cntr_V_dim}
     \end{subfigure}
\caption{
Different downstream functional family $\Qpred$ require
(a) corresponding or larger functional family during ISSL $\Qpred \subseteq \Qissl $;
(b) smaller dimensionality of $Z$ when $\Q$ is larger.
3 seeds.
Same as \cref{fig:func_family} but with contrastive learning and downstream predictors are evaluated on unseen test examples, \ie, without assuming knowledge of $p(X)$ during ISSL.
}
\label{fig:cntr_func_family}
\vspace{-0.5em}
\end{figure}

==> figures/controlled/regularization.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[t]{0.4\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/controlled/reg_dim.pdf}
         \caption{Dimensionality}
         \label{fig:reg_dim}
     \end{subfigure}
     \begin{subfigure}[t]{0.4\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/controlled/reg_samples.pdf}
         \caption{Sample efficiency}
         \label{fig:reg_samples}
     \end{subfigure}
%\vspace{-0.3em}
\caption{
Regularizers that ensure that equivalent examples are mapped to the same representations are necessary to achieve the minimal required (a) dimensionality $d(\Q)$; and (b) sample efficiency $\rS{}$. 
Longer training is an implicit such regularizer.
3 seeds.
}
\label{fig:regularizers}
\vspace{-0.5em}
\end{figure}

==> figures/mnist/effect_n_tasks.tex <==
\begin{figure}[h]
     \centering
     \includegraphics[width=\linewidth]{figures/mnist/lines_acc_vs_agg.pdf}
\caption{
Effect of approximations for computing $\sup_y$ in \tocref{}.
X axis shows the number of random subtasks that are considered (log axis). 
Y axis shows the estimated $\sup_y \Risk{M(X)}{Z}$. The style of the line shows which tasks are considered (binary or all).
``Contrastive'' and ``generative'' are our ISSL methods, while ``std contr.'' and ``std gen.'' are their standard counterparts.
}
\label{fig:effect_n_tasks}
\vspace{-0.5em}
\end{figure}

==> figures/schemas/Mx/Mx.tex <==
\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-rotation.pdf}
         \caption{Radius for \\ rotation invariance.}
         \label{fig:Mx_rotation}
     \end{subfigure}
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-permutation.pdf}
         \caption{Histogram for \\ permutation Invariance.}
         \label{fig:Mx_permutation}
     \end{subfigure}
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-augmentations.pdf}
         \caption{Unaugmented $X$ for \\
         augmentation invariance.}
         \label{fig:Mx_augmentation}
     \end{subfigure}
\vspace{-0.3em}
\caption{
Maximal invariants $M(X)$ are representatives of equivalence classes. The figure shows examples of $M(X)$ and is modified with permission from \citet{dubois_lossy_2021}.
}
\label{fig:max_inv}
\vspace{-0.5em}
\end{figure}

==> figures/schemas/Mx/aug_Mx.tex <==
\begin{wrapfigure}{r}{0.43\textwidth}
\vspace{-1.7\baselineskip}
 \centering
 \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-augmentations.pdf}
\caption{

$M(X)$ are representatives of equivalence classes. Modified from \cite{dubois_lossy_2021}.
}
\label{fig:max_inv}
\vspace{-1.5em}
\end{wrapfigure}


==> figures/schemas/Mx/wrap_Mx.tex <==
\begin{wrapfigure}{r}{0.43\textwidth}
\vspace{-1.7\baselineskip}
\centering
     \centering
     \begin{subfigure}[t]{0.47\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-rotation.pdf}
         \vspace*{-1.5em}
         \caption{Radius for \\ rotation invariance.}
         \label{fig:Mx_rotation}
     \end{subfigure}
    %  \begin{subfigure}[t]{0.325\linewidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-permutation.pdf}
    %      \caption{Histogram for \\ permutation Invariance.}
    %      \label{fig:Mx_permutation}
    %  \end{subfigure}
     \begin{subfigure}[t]{0.515\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/Mx/max_invariants-augmentations.pdf}
         \vspace*{-1.5em}
         \caption{Unaugmented $X$ for
         augment. invariance.}
         \label{fig:Mx_augmentation}
     \end{subfigure}
%\vspace{-0.3em}
\caption{
$M(X)$ are representatives of equivalence classes. Modified from \cite{dubois_lossy_2021}.
}
\label{fig:max_inv}
\vspace{-1.5em}
\end{wrapfigure}


==> figures/schemas/aug/aug.tex <==
\begin{figure}[t!]
     \centering
     \begin{subfigure}[t]{0.47\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/aug/Aug_Mx.pdf}
         \caption{$\RiskA{M(X)}{Z}$.}
         \label{fig:aug_mx}
     \end{subfigure}
     \begin{subfigure}[t]{0.47\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/aug/Aug_A.pdf}
         \caption{$\RiskA{A}{Z}$.}
         \label{fig:aug_A}
     \end{subfigure}
\vspace{-0.3em}
\caption{
Encoders that minimize $\RiskA{A}{Z}$ with shattering also minimize the desired $\distsA{}$, as long as the kernel of the Bayes predictor $\sim_A$ is a refinement of the desired equivalence $\sim$.
}
\label{fig:aug}
\vspace{-0.5em}
\end{figure}

==> figures/schemas/geometry/geometry_old.tex <==
\ydnote{Is this figure understandable without reading the text? }
\begin{figure}[h]
     \centering
     \begin{subfigure}{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/geometry/Geometry Zb.pdf}
         \SmallCaption{No pred. of $M(X)$}
         \label{fig:geometry_zb}
     \end{subfigure}
     \begin{subfigure}{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/geometry/Geometry Zu.pdf}
         \SmallCaption{$\U$ pred. of $M(X)$}
         \label{fig:geometry_zu}
     \end{subfigure}
     \begin{subfigure}{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/geometry/Geometry Zl.pdf}
         \SmallCaption{$\Q$ pred. of $M(X)$}
         \label{fig:geometry_zl}
     \end{subfigure}
     \begin{subfigure}{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/geometry/Geometry Zns.pdf}
         \SmallCaption{Task $t \in \tasksinv{}$ not $\Q$ pred.}
         \label{fig:geometry_zns}
     \end{subfigure}
     \begin{subfigure}{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/schemas/geometry/Geometry Zs.pdf}
         \SmallCaption{$\Q$ pred. and high dim.}
         \label{fig:geometry_zs}
     \end{subfigure}
\caption{
An encoder is population optimal for linear $\Q$ if and only if it allows linear prediction of a maximal invariant $M(X)$ and the dimensionality is large enough. (a) Universal predictability is necessary but (b) not sufficient for linear predictability. (c) Linear predictability of $M(X)$ does (d) not ensure predictability of all invariant task; besides iff (e) the dimensionality is at least $\nequiv -1$.
}
  \label{fig:geometry}
\vspace{-0.5em}
\end{figure}


% An encoder is optimal for linear $\Q$ if and only if it allows linear prediction of a maximal invariant $M(X)$, its dimensionality is large enough, and is invariant. (a) Universal separability is not sufficient for linear separability. (b) Linear separability of $M(X)$ does (c) not ensure linear separability of all invariant task; besides iff (d) the dimensionality is at east $\nequiv -1$. (e) For sample optimality 

==> figures/schemas/losses/dissl.tex <==
\begin{wrapfigure}{r}{0.25\textwidth}
\vspace*{-4.2em}
\centering
 \centering
 \includegraphics[width=\linewidth]{figures/schemas/losses/ISSL_objectives-dissl-cropped.pdf}
\caption{
DISSL}
\label{fig:dissl}
\vspace*{-2em}
\end{wrapfigure}


==> figures/schemas/losses/losses.tex <==
\begin{figure}[h]
 \centering
 \includegraphics[width=0.7\linewidth]{figures/schemas/losses/selfdistil.pdf}
 \label{fig:self_distil}
\vspace*{-2em}
\caption{
Self distillation loss.
}
\vspace*{-2em}
\label{fig:sample}
\end{figure}

==> figures/schemas/losses/objectives.tex <==

\begin{figure}[t]
\centering
 \begin{subfigure}[t]{0.32\linewidth}
     \centering
     \includegraphics[width=\linewidth]{figures/schemas/losses/ISSL objectives-cissl.pdf}
     \caption{CISSL}
     \label{fig:CISSL}
 \end{subfigure}
  \begin{subfigure}[t]{0.3\linewidth}
     \centering
     \includegraphics[width=\linewidth]{figures/schemas/losses/ISSL objectives-dissl.pdf}
     \caption{DISSL}
     \label{fig:DISSL}
 \end{subfigure}
 \begin{subfigure}[t]{0.21\linewidth}
     \centering
     \includegraphics[width=\linewidth]{figures/schemas/losses/ISSL objectives-gissl.pdf}
     \caption{GISSL}
     \label{fig:GISSL}
 \end{subfigure}
 \caption{Our objectives for linear probing $\Q$: $\mathrm{softmax}({\color{royalblue}{W}}^T{\color{Orange}{z}})[Y]$.}
 \label{fig:objectives_issl}
%
\end{figure}

==> figures/schemas/objective.tex <==
\begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{figures/schemas/objectives-full.pdf}
\caption{
Illustration of one of our proposed objective (invariant VAE), for invariances w.r.t. image augmentation.
We minimize the \textcolor{bluedark}{rate} using a KL divergence between the marginal and a prior.
The \textcolor{burntorange}{distortion} is minimized by reconstructing unaugmented images.
All our objectives have the same intuition, but use different methodologies. 
See \cref{fig:distortions} for more distortions.
}
\label{fig:objective}
\vspace{-0.5em}
\end{figure}

==> figures/schemas/setting/setting.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace*{-2em}
\centering
 \centering
 \includegraphics[width=\linewidth]{figures/schemas/setting/issl_setting_groupc.pdf}
\caption{
Summary of ISSL setting and notation.
}
\label{fig:setting}
\vspace*{-1.5em}
\end{wrapfigure}


==> figures/schemas/summary/optimal_representation.tex <==
\begin{wrapfigure}{r}{0.31\textwidth}
\vspace*{-2.7em}
\centering
 \centering
 \includegraphics[width=\linewidth]{figures/schemas/summary/optimal_representation.pdf}
\caption{
Optimal representations for linear probes ensure perfect linear predictors on augmentation invariant tasks.
}
\label{fig:optimal_rep}
\vspace{-1.5em}
\end{wrapfigure}


==> figures/schemas/summary/wrap_summary.tex <==
\begin{wrapfigure}{r}{0.26\textwidth}
\vspace*{-1em}
\centering
 \centering
 \includegraphics[width=\linewidth]{figures/schemas/summary/minimal_sufficient_task.pdf}
\caption{
There exists a pretext task $M(X)$ that ensures prediction of all invariant task including those of interest.
}
\label{fig:optimal_rep}
\vspace{-1.5em}
\end{wrapfigure}


==> figures/schemas/venn.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/schemas/venn_diagram-Y.pdf}
         \caption{$\rv X$ and labels of interest $\Yt$}
         \label{fig:venn_diagram_y}
     \end{subfigure}
     \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/schemas/venn_diagram-Z.pdf}
         \caption{Representation $\rv Z$}
         \label{fig:venn_diagram_z}
     \end{subfigure}
     \begin{subfigure}[t]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/schemas/venn_diagram-invariance.pdf}
         \caption{$\mathcal{G}$-invariance requirement}
          \label{fig:venn_diagram_invariant}
     \end{subfigure}
\caption{Information diagram showing: a) the difference between the current compression that need at least ${ \color{bluedark} \op{H}{\rv X}}$ bit and the best possible compression (for predicting ${ \color{golddark} \Yt{} }$) which only needs ${ \color{greendark} \IXYt{}}$ bits. 
b) The representation ${ \color{reddark} \rv Z}$ that we are aiming to learn (as we assumed that we cannot directly access ${ \color{golddark} \Yt{} }$), it  only requires ${ \color{purpledark} \MI{X}{Z}}$ bits for transmission but still has all the desired information $\op{I}{ { \color{golddark} \Yt{} } ; { \color{reddark} \rv Z } }= { \color{greendark} \IXYt{}}$. 
c) Our approach to learning a ``good'' $\rv Z$ by finding properties that are satisfied by all tasks of interest ${ \color{golddark} \Yt{} }$, as a result we will be able to remove information in ${ \color{bluedark} \rv X}$ about tasks that do not satisfy these properties, giving a gain of $\op{H}{ \color{graydark} \set{ \rv Y \cond \rv Y \text{ does not satisfy properties of interest} } }$ bits. 
The desired properties will be formalized using group theory.
}
\label{fig:venn_diagram}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/acc.tex <==
\begin{table}[h]
\caption{\tofill{}
}
\label{tab:acc}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllrr}
\toprule
Mode & $\Q$ & Aug.& Reg.  & Worst Acc. &  Acc.   \\
\midrule
C  & L &  inv. & $\times$ &  &  \\
\textcolor{orange}{C} & L &   inv. & $\surd$ &  &    \\
C  & L &   & $\times$ &  &  \\
\textcolor{orange}{C}   & L &    & $\surd$ & &  \\
C  & L &  cov. & $\surd$ &  &  \\
\textcolor{orange}{C}   & L &   cov. & $\times$ &  &  \\
\textcolor{orange}{C}  & M &   inv. & $\times$ &  & \\
D & L &  inv. & $\times$ &  & \\
\textcolor{orange}{D}  & L &   inv. & $\surd$ &  & \\
D  & M &   inv. & $\times$ & &  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/controlled/appcs/cntr_permMx.tex <==
\begin{table}[h]
\caption{
Permuting $M(X)$ has little effect on contrastive ISSL on CIFAR10.
E.g., predicting ``$(n+1)\%10$'' for all images of digits of ``$n$''. 3 seeds.
}
\label{tab:cntr_permMX}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrr}
\toprule
 & $\RiskA{M(X)}{Z}$ & $\sup_Y \RiskA{Y}{Z}$ \\
\midrule
$M(X)$ &  $83.44 \pm 0.24$ &  $88.51 \pm 0.08$ \\
Permuted $\pi(M(X))$  &   $82.97 \pm 0.29$ &  $88.27 \pm 0.30$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}
%
% \begin{table}[h]
% \caption{
% Permuting $M(X)$ has little effect on contrastive ISSL on CIFAR10.
% E.g., predicting ``$(n+1)\%10$'' for all images of digits of ``$n$''. 3 seeds.
% }
% \label{tab:cntr_permMX}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrrr}
% \toprule
%  & \multicolumn{2}{c}{$\RiskA{M(X)}{Z}$} & \multicolumn{2}{c}{$\sup_Y \RiskA{Y}{Z}$} \\
%  &  Train & Test  & Train & Test \\
% \midrule
% $M(X)$ & $100.00 \pm 0.00$ & $83.44 \pm 0.24$ & $99.99 \pm 0.00$ & $88.51 \pm 0.08$ \\
% Permuted $\pi(M(X))$  & $99.96 \pm 0.01$ &  $82.97 \pm 0.29$ & $99.94 \pm 0.03$ & $88.27 \pm 0.30$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

==> tables/controlled/appcs/exact_losses.tex <==
\begin{table}[h]
\caption{
The loss used during (exact) ISSL on CIFAR10 has little effect on downstream performance regardless of downstream losses. 3 seeds. Showing $\sup_Y \RiskA{Y}{Z}$ on train.
}
\label{tab:exact_losses}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
 \diagbox{ISSL}{Pred.}  & Log. Loss & Hinge & MSE & 0-1 \\
\midrule
Log. Loss & $0.000 \pm 0.000$ & $0.000 \pm 0.000$  & $0.011 \pm 0.001$  & $0.000 \pm 0.000$ \\
Hinge & $0.002 \pm 0.000$ & $0.000 \pm 0.000$  & $0.009 \pm 0.001$  & $0.000 \pm 0.000$ \\
MSE & $0.001 \pm 0.000$ & $0.000 \pm 0.000$  & $0.000 \pm 0.000$  & $0.000 \pm 0.000$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/controlled/appcs/exact_losses_test.tex <==
\begin{table}[h]
\caption{
The loss used during (exact) ISSL on CIFAR10 can have effect effect on downstream performance when considering finite sample generalization. 3 seeds. 
Showing $\sup_Y \RiskA{Y}{Z}$ on test.
}
\label{tab:exact_losses_test}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
 \diagbox{ISSL}{Pred.}  & Log. Loss & Hinge & MSE & 0-1 \\
\midrule
Log. Loss & $0.419	 \pm 0.008$ & $0.220 \pm 0.005$  & $0.272 \pm 0.005$  & $0.092 \pm 0.002$ \\
Hinge & $0.338 \pm 0.006$ & $0.238 \pm 0.004$  & $0.300 \pm 0.004$  & $0.102 \pm 0.002$ \\
MSE & $0.492 \pm 0.011$ & $0.212 \pm 0.005$  & $0.291 \pm 0.004$  & $0.093 \pm 0.002$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/controlled/appcs/exact_permMx.tex <==
\begin{table}[h]
\caption{
Permuting $M(X)$ has little effect on exact ISSL.
E.g., predicting ``$(n+1)\%10$'' for all images of digits of ``$n$''. 3 seeds.
}
\label{tab:exact_permMX}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrr}
\toprule
 & $\RiskA{M(X)}{Z}$ & $\sup_Y \RiskA{Y}{Z}$ \\
\midrule
$M(X)$ & $100.00 \pm 0.00$  &$100.00 \pm 0.00$ \\
Permuted $\pi(M(X))$  & $100.00 \pm 0.00$  &$100.00 \pm 0.00$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}
% \begin{table}[h]
% \caption{
% Permuting $M(X)$ has little effect on exact ISSL.
% E.g., predicting ``$(n+1)\%10$'' for all images of digits of ``$n$''. 3 seeds.
% }
% \label{tab:exact_permMX}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrrr}
% \toprule
%  & \multicolumn{2}{c}{$\RiskA{M(X)}{Z}$} & \multicolumn{2}{c}{$\sup_Y \RiskA{Y}{Z}$} \\
%  &  Train & Test  & Train & Test \\
% \midrule
% $M(X)$ & $100.00 \pm 0.00$ & $86.85 \pm 0.11$ &$100.00 \pm 0.00$ &  $90.89 \pm 0.36$\\
% Permuted $\pi(M(X))$  & $100.00 \pm 0.00$ & $86.90 \pm 0.22$ &$100.00 \pm 0.00$ & $90.85 \pm 0.39$\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \end{table}

==> tables/controlled/appcs/mnist.tex <==
\begin{table}[h]
\caption{Comparing different ISSL methods in MNIST controlled experiments. 3 seeds.
}
\label{tab:appcs:mnist}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llrrrrrr}
\toprule
& & $\rS{}$ & $d(\Q)$ &  $\RiskA{M(X)}{Z}$  train & $\RiskA{M(X)}{Z}$  & $\sup_Y \RiskA{Y}{Z}$  & 100 labels \\
\midrule
& Supervised & 10000 &  &  $100.00 \pm 0.00$  & $99.59 \pm 0.02$ & $99.20 \pm 0.00$  & $38.89 \pm 3.66$ \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize  \centering ~Exact  }}  
& Ours & $\times$ & $\times$ & $97.46 \pm 0.02$ & $97.42 \pm 0.05$ & $96.09 \pm 0.24$ & $73.77 \pm 2.02$ \\
& \quad $\Q$ & $\times$ & $\times$ & $97.11 \pm 0.31$ & $97.36 \pm 0.26$ & $96.51 \pm 0.20$ & $81.60 \pm 2.06$ \\
& \quad $\Q^+$ & $\times$ & $\times$ & $97.11 \pm 0.26$ & $97.33 \pm 0.27$ & $96.18 \pm 0.14$ & $85.05 \pm 1.44$ \\
 \cmidrule{2-8}
& \quad  opt. aug. & 10 & $\times$ 10 & $100.00 \pm 0.00$  &  $99.52 \pm 0.03$  &  $99.56 \pm 0.02$ & $99.43 \pm 0.02$ \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Generative  }}  
& Standard & $\times$ &$\times$  & $93.03 \pm 0.15$ & $93.41 \pm 0.17$ & $83.74 \pm 0.90$   & $77.75 \pm 0.62$ \\
 & Ours & 10000 & 2048 & $99.74 \pm 0.00$ & $99.15 \pm 0.01$ & $98.64 \pm 0.11$ & $87.32 \pm 0.04$ \\  
& \quad $\Q$ & $\times$ & $\times$ & $95.39 \pm 0.03$ & $95.66 \pm 0.01$ & $94.02 \pm 0.71$ &   $77.85 \pm 0.13$ \\
& \quad $\Q^+$ & 10000 & $\times$ & $99.76 \pm 0.01$ & $99.30 \pm 0.04$ & $98.56 \pm 0.06$ &  $90.48 \pm 1.43$ \\
& \quad reg. & 10000 & 2048 & $99.53 \pm 0.01$ & $99.25 \pm 0.02$ & $98.56 \pm 0.05$ & $88.48 \pm 0.29$ \\
 \cmidrule{2-8}
& \quad opt. aug. & 10 &10 &  $99.97 \pm 0.01$ & $99.64 \pm 0.01$ & $99.74 \pm 0.11$ & $99.63 \pm 0.02$ \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize  \centering ~Contrastive  }} 
& Standard & 10000 & 2048 & $99.51 \pm 0.00$ &  $99.34 \pm 0.05$  & $98.40 \pm 0.11$ & $92.02 \pm 0.84$ \\
 & Ours & 10000 & 512 & $\mathbf{99.80} \pm 0.00$ &  $99.28 \pm 0.03$  & $98.87 \pm 0.05$ & $86.00 \pm 0.31$ \\
& \quad $\Q$ & 10000 & $\times$ & $99.73 \pm 0.02$ &  $99.29 \pm 0.04$  & $\mathbf{98.90} \pm 0.04$ & $84.90 \pm 0.13$ \\
& \quad $\Q^+$ & 10000 & 2048 & $99.52 \pm 0.03$ &  $99.30 \pm 0.02$  & $98.62 \pm 0.06$ & $90.50 \pm 1.38$ \\
& \quad reg. & 10000 & 512 & $99.67 \pm 0.01$ &  $\mathbf{99.35} \pm 0.03$  & $98.79 \pm 0.12$ & $87.13 \pm 0.23$ \\
 \cmidrule{2-8}
& \quad opt. aug. & 10 & 10 & $100.00 \pm 0.00$ &  $99.57 \pm 0.02$ & $99.59 \pm 0.03$ & $99.54 \pm 0.02$ \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize  \centering ~Self-Dist.  }} 
& Standard & $\times$ & $\times$ & $91.65 \pm 0.94$ &  $92.12 \pm 0.80$  & $92.60 \pm 0.84$ &  $77.93 \pm 2.33$ \\
 & Ours & 10000 & 32 & $98.91 \pm 0.31$ &  $98.93 \pm 0.30$  & $98.69 \pm 0.43$ & $91.26 \pm 4.42$ \\
& \quad $\Q$ & 10000 & $\times$  & $99.08 \pm 0.06$ &  $99.11 \pm 0.04$  & $98.77 \pm 0.03$ &  $93.77 \pm 0.22$ \\
& \quad $\Q^+$ & 10000 & 512 & $99.08 \pm 0.06$ &  $99.21 \pm 0.03$  & $98.88 \pm 0.08$ & $95.47 \pm 0.50$ \\
& \quad reg. & 10000 & 128 & $98.95 \pm 0.08$ &  $99.07 \pm 0.07$  & $\mathbf{98.90} \pm 0.15$ & $\mathbf{95.68} \pm 0.28$ \\
 \cmidrule{2-8}
& \quad opt. aug. & 100 & 16 & $99.91 \pm 0.06$ & $99.49 \pm 0.03$  & $99.84 \pm 0.08$ & $96.92 \pm 1.57$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> tables/controlled/appcs/mnist_dim.tex <==
\begin{table}[h]
\caption{
The optimal required dimensionality can essentially be achieved by all approximate ISSL objectives. 
$d(\Q)$ is estimated by sweeping over dimensions and looking at the minimal dimension that achieves $98\%$
downstream accuracy. 3 seeds.
}
\label{tab:appcs:aug_dim}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
&  Exact & Generative  & Contrastive  & 
Self-Dist.\\
\midrule
Std. Aug. & $\times$ & 2048 & 512  & 32    \\
Opt. Aug. & 10 & 10  & 10 & 16    \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}


==> tables/controlled/appcs/mnist_samples.tex <==
\begin{table}[h]
\caption{
The optimal sample efficiency can essentially be achieved by all approximate ISSL objectives. 
$\rS{}$ is estimated by sweeping over dimensions and looking at the minimal number of downstream training samples to achieves $98\%$
downstream accuracy. 3 seeds.
}
\label{tab:appcs:aug_dim}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
&  Exact & Generative  & Contrastive  & 
Self-Dist.\\
\midrule
Std. Aug. &   $\times$ & 10000 & 10000  & 10000    \\
Opt. Aug. & 10 & 10  & 10 & 100    \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}


==> tables/controlled/main/losses.tex <==
\begin{table}[h]
\caption{\tofill{}
}
\label{tab:acc}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrr}
\toprule
 & MNIST & Tiny Imagenet   \\
\midrule
Gen. base & \hyp{$90\%$} & \hyp{$30\%$}   \\
Gen. ours & \hyp{$95\%$} & \hyp{$35\%$}   \\
\midrule
Cont. base & \hyp{$94\%$} & \hyp{$50\%$}   \\
Cont. ours & \hyp{$96\%$} & \hyp{$52\%$}   \\
Cont. ours batch $\searrow$ & \hyp{$80\%$} & \hyp{$40\%$}   \\
\midrule
Self-Dis. base & \hyp{$94\%$} & \hyp{$50\%$}   \\
Self-Dis. ours & \hyp{$98\%$} & \hyp{$54\%$}   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/controlled/main/regularization.tex <==
\begin{table}[h]
\caption{Regularization is necessary to achieve the minimal dimension and sample efficiency. 3 seeds.
}
\label{tab:acc}
%\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrr}
\toprule
 & Dim. $d(\Q)$ & Sample eff. $\rS$   \\
\midrule
Regularized & \textbf{$10$} & $10$   \\
Not Reg. & $256$ & $64$   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
%\vskip -0.1in
\end{table}

==> tables/pretrained/losses.tex <==
\begin{table}[h]
\caption{
The loss used during ISSL is unrelated to the downstream predictive loss. 3 seeds. 
}
\label{tab:pretrained_loss}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrrr}
\toprule
 \diagbox{ISSL}{Pred.}  & Log. Loss & MSE & 0-1 \\
\midrule
log loss  &  &  &  \\ %(simclr / swav / dino)
MSE  &  &  &  \\ %(byol / simsiam)
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/pretrained/pretrained.tex <==
\begin{table*}[h]
\caption{Standard pretrained SSL models follow our theory despite approximations}
\label{tab:pretrained}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lllrrrr}
\toprule
 & Aug. & Dim. &  $\RiskA{M(X)}{Z}$ Train & $\RiskA{M(X)}{Z}$ & $\sup_Y \RiskA{Y}{Z}$ & $\rS{}$   \\
\midrule
DINO & Fine & ? & & & &  \\
SwAV & Fine & ? & & & &  \\
SimCLR & Fine & ? & & & &  \\
CLIP & coarse & ? & & & &  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/realistic/appcs.tex <==
\begin{table}[h]
\caption{Comparing different our and standard approximation of the ISSL objective on CIFAR10. 3 seeds.
}
\label{tab:appcs:mnist}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llrrrr}
\toprule
& &  $\sup_Y \RiskA{Y}{Z}$   & $1\%$  &  $10\%$ & $100\%$\\
% & &  $\sup_Y \RiskA{Y}{Z}$   &   \multicolumn{3}{c}{$\RiskA{M(X)}{Z}$} \\
% & &  & $1\%$  &  $10\%$ & $100\%$\\
\midrule
& Supervised & & & & \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Generative  }}  
& Std. & & & & \\
& \quad $\Q^+$ & & & & \\
& Ours & & & & \\
& \quad $\Q^+$ & & & & \\
& \quad Reg. & & & & \\
& \quad Dim. $\nearrow$ & & & & \\
 \cmidrule{2-6}
& \quad opt. aug. & & & & \\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Contrastive  }}  
& Std. & & & & \\
& \quad $\Q^+$ & & & & \\
& Ours & & & & \\
& \quad $\Q^+$ & & & & \\
& \quad Reg. & & & & \\
& \quad Dim. $\nearrow$ & & & & \\
& \quad Batch $\nearrow$ & & & & \\
 \cmidrule{2-6}
& \quad opt. aug. & & & & \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Self-Distillation  }}  
& Std. & & & & \\
& \quad $\Q^+$ & & & & \\
& Ours & & & & \\
& \quad $\Q^+$ & & & & \\
& \quad Reg. & & & & \\
& \quad Dim. $\nearrow$ & & & & \\
 \cmidrule{2-6}
& \quad opt. aug. & & & & \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> tables/realistic/main.tex <==
\begin{figure}[t]
%\centering
\begin{minipage}{.55\linewidth}
\captionof{table}{Our theoretical insights improve all types of ISSL on TinyImagenet.  Linear and MLP probes $\Q$ trained on all or $1\%$ train data.  Top-1 acc. 3 seeds.}
\label{tab:tinyimagenet}
\begin{center}
\begin{small}
\begin{tabular}{llrrr}
\toprule
&&  \multicolumn{2}{c}{ Linear $\Q$}  & MLP $\Q^+$  \\
\cmidrule(lr){3-4} \ 
&&  All &  5-shot & All  \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ \footnotesize \centering ~Gen.  }}
&  AE   & $9.8$ {\tiny $\pm 0.1$}  & &  \\
&  VAE   & $12.3$ {\tiny $\pm 0.2$}  & $1.8$ {\tiny $\pm 0.2$} &  \\
\cmidrule{2-5}
& \textbf{GISSL} {\tiny (ours)}    & $\mathbf{21.3}$ {\tiny $\pm 0.3$} & &  \\
& \ + dim $\uparrow$   &  &   &   \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Cntr.  }}  
& SimCLR & $44.6$ {\tiny $\pm 0.3$} & $16.6$ {\tiny $\pm 0.1$} & $46.3$ {\tiny $\pm 0.1$} \\
\cmidrule{2-5}
& \textbf{CISSL}  {\tiny (ours)}  & $\mathbf{45.3}$ {\tiny $\pm 0.2$} & $\mathbf{17.5}$ {\tiny $\pm 0.0$} & 
$\mathbf{46.8}$ {\tiny $\pm 0.2$}
\\
& \ + dim $\uparrow$   & $\mathbf{51.3}$  {\tiny $\pm 0.1$}  &   &   \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ \footnotesize \centering ~Distil.  }} 
& SwAV & $40.3$ {\tiny $\pm 0.2 $} &$ \mathbf{19.5} $ {\tiny $\pm 0.3 $}  & $ 40.7 $ {\tiny $\pm 0.1 $} \\
%& SimSiam & $40.1$ {\tiny $\pm 0.3$} &$16.2$ {\tiny $\pm 0.4$}  & $46.0$ {\tiny $\pm 0.1$} \\
& DINO & $43.3$ {\tiny $\pm 0.3$} & $17.9$ {\tiny $\pm 0.3$} & $44.2$ {\tiny $\pm 0.4$} \\
%& SimSiam & $42.8$ {\tiny $\pm 0.3$} &  &  \\
\cmidrule{2-5}
& \textbf{DISSL} {\tiny (ours)}  & $\mathbf{44.9}$ {\tiny $\pm 0.1$} & $18.6$ {\tiny $\pm 0.0$} &  $\mathbf{45.6}$ {\tiny $\pm 0.2$} \\
& \ + dim $\uparrow$   & $\mathbf{47.0}$  {\tiny $\pm 0.1$} &   &   \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{minipage}
\end{figure}

==> tables/scaled/imagenet_mlp.tex <==
\begin{figure}[h]
%\centering
\begin{minipage}{.39\linewidth}
\captionof{table}{MLP $\Q$. }
\label{tab:mlp}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrr}
\toprule
& All & 10 shot \\
\midrule
Linear DISSL & \seeds{44.0} & \seeds{21.7}  \\
\midrule
Naive DINO & \seeds{42.4}  &  \seeds{19.0} \\
Naive DISSL & \run{?}  & \run{?}  \\
\midrule
MLP DISSL & \rerun{45.2} & \rerun{22.0}  \\
%Supervised \cite{ermolov_whitening_2021} &  &  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{minipage}
%
\hfill{}
\begin{minipage}{.5\linewidth}
\captionof{table}{
We outperform SWAV on ImageNet.}
\label{tab:imagenet}
\begin{center}
\begin{small}
\begin{tabular}{lrrrr}
\toprule
&&  \multicolumn{2}{c}{ Linear $\Q$}  & MLP $\Q^+$  \\
\cmidrule(lr){3-4}\
&&  100 ep. &  400 ep. & 100 ep.  \\
\midrule
 & SwAV  & \rerun{66.8}  & \rerun{70.2 } & \run{?} \\
& \textbf{DISSL} {\tiny (our)}  & \rerun{67.2} &  \rerun{70.1} &  \run{?}  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{minipage}
%
\end{figure}


% \begin{figure}[h]
% %\centering
% \begin{minipage}{.7\linewidth}
% \captionof{table}{
% We outperform SimCLR and SWAV on ImageNet.}
% \label{tab:imagenet}
% \begin{center}
% \begin{small}
% \begin{tabular}{llrrrr}
% \toprule
% &&  \multicolumn{2}{c}{ Linear $\Q$}  & MLP $\Q^+$  \\
% \cmidrule(lr){3-4}\
% &&  100 ep. &  400 ep. & 100 ep.  \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Cntr  }} & SimCLR  & &   \\
% & \textbf{CISSL} {\tiny (our)}  & & &  \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\scriptsize \centering ~Dist  }} & SwAV  & & &  \\
% & \textbf{SISSL} {\tiny (our)}  & & &  \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{minipage}
% \end{figure}

==> tables/toy.tex <==
\begin{table}[h]
\caption{Toy experiments.
``Mode'' says whether we use contrastive ``C'' or direct ``D'' loss.
``inv.'' or ``cover'' mean that the augmentation satisfies $A(X) \indep X \cond M(X)$, or $\mathcal{G}_{A}(X) = [X]$ respectively.
$\mathcal{F}$ says whether using linear ``L'' or MLP ``M'' predictor.
``Reg'' says whether we use $\KL{p(Z|X),p(Z|\Tilde{X})}$ regularizer.
$\hat{d}$ is an empirical estimate of the necessary dimension to perform invariant tasks.
$\hat{S}$ is an empirical estimate of the necessary number of downstream samples to perform invariant tasks.
``Acc.'' uses $d=10,S=1000$ and evaluates accuracy on test set.
}
\label{tab:toy}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llllrrr}
\toprule
Mode & $\Q$ & Aug.& Reg.  & { \scriptsize $\RiskA{M(X)}{Z}$ }  & $\hat{d}$ & $\hat{S}$    \\
\midrule
C  & L &  $\times$ & $\times$ & \hyp{$10\%$} &  &  \\
C  & L &  inv. & $\times$ & \hyp{$100\%$} & \hyp{9} & \hyp{50}  \\
\textcolor{orange}{C} & L &   inv. & $\surd$ & \hyp{$100\%$} &\hyp{9} & \hyp{50}   \\
C  & L &   & $\times$ &\hyp{$100\%$} & \hyp{500} & \hyp{9000}  \\
\textcolor{orange}{C}   & L &    & $\surd$ & \hyp{$100\%$} &\hyp{300} & \hyp{3000}  \\
C  & L &  cov. & $\surd$ & \hyp{$100\%$} &\hyp{9} & \hyp{50} \\
\textcolor{orange}{C}   & L &   cov. & $\times$ & \hyp{$100\%$} &\hyp{500} & \hyp{9000} \\
\textcolor{orange}{C}  & M &   inv. & $\times$ & \hyp{$100\%$} &\hyp{3} & \hyp{500}  \\
D & L &  inv. & $\times$ & \hyp{$100\%$} &\hyp{9} & \hyp{50} \\
\textcolor{orange}{D}  & L &   inv. & $\surd$ & \hyp{$100\%$} &\hyp{9} & \hyp{50} \\
D  & M &   inv. & $\times$ & \hyp{$100\%$} &\hyp{3} & \hyp{500}  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> text/approximation_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Approximating ISSL Objectives in practice}
% \label{sec:objective}

In previous sections, we showed that encoders are discriminative and sample efficient iff they
\begin{inlinelist}
\item minimize $\Risk{\Mx{A}(X)}{Z}$;
\item are $\sima$-shatterable;
\item yield invariant representations.
\end{inlinelist}
The question then becomes how to practically enforce those properties.
Here we focus on (i), specifically, we derive different ISSL objectives approximating $\Risk{\Mx{A}(X)}{Z}$.
In the process we shed light as to why previously proposed ISSL methods and tricks work, and how to improve them in practice.

For space constraints we consider (ii) and (iii) in \cref{sec:appx:derivations}. 
For (ii) we show that $\sim$-shatterability holds with high $p$ when the effective dimensionality satisfies \cref{cor:dimension}.
For (iii) we discuss regularizers for invariance.
Both properties should be more thoroughly investigated in future work.


To improve the section's practicality, %and understandability
we focus on typical ISSL settings. 
For more general cases, derivations, pseudocode see \cref{sec:appx:derivations}.
Specifically, in the main paper, we consider: a deterministic encoder $Z = Z_{\theta}(X)$,  predictors $f \in \Q$ that decompose $f(Z) = W^T h_{\phi}(Z)$ into a specific hidden component $h_{\phi}$ and any linear layer $W \in \mathbb{R}^{d \times |\Yc|}$ to logits, and a surrogate log-softmax loss $\ell(Y,f(Z)) = - \log \mathrm{softmax}(f(Z))[Y]$ where $[Y]$ denotes vector indexing.
We will use $\phi \in \Phi$ to remember that $h_{\phi}$ is constrained by $\Q$, \eg, if $\Q$ are linear predictors with no bias, then $h_{\phi}$ must be the identity so that $\Q \defeq \set{ f : Z \mapsto W^T Z}$. 
The objective to approximate is then:
%
\begin{equation}\label{eq:obj_to_appx}
%\Risk{\Mx{A}}{Z_{\theta}} \defeq  \inf_{\phi \in \Phi, W} \Ep{\p{X}}{- \log \frac{\exp{ \pa{ W[\Mx{A}] ^T h_{\phi}(Z_{\theta})} } }{ \sum_{m} \exp{ \pa{ W[m] ^T h_{\phi}(Z_{\theta})} } }}, = \inf_{W,\phi} \Ep{\p{X}}{- \log q_{\scriptsriptstyle W,\phi}(\Mx{A} \cond Z_{\theta})},
\Risk{\Mx{A}}{Z_{\theta}} \defeq  \inf_{\phi \in \Phi, W} \Ep{\p{X}}{- \log \frac{\exp{ \scores{}(\Mx{A},Z_\theta) } }{ \sum_{m} \exp{ \scores{}(m,Z_\theta) } }}, 
\quad  \scores{}(m,z) \defeq W[m] ^T h_{\phi}(z)
\end{equation}
% 
where the sum is over classes $m \in 1, \dots, \nequiva{}$, we distributed indexing inside the softmax, we use the shorthands $\Mx{A} \defeq \Mx{A}(X)$,  $Z_{\theta} \defeq Z_{\theta}(X)$, and use $\scorew{}(m,z)$ for the m\textsuperscript{th} logit.
The difficulty with \cref{eq:obj_to_appx} is that we do know the maximal invariant $\Mx{A}$ or ways of enumerating equivalence classes. 
We consider three classes of methods to solve this: contrastive, self-distillation, and generative.
In each, we only assume access to an augmentor $\augmentor{}(\Tilde{X} | X)$ to equivalent examples $\Tilde{X} \sima X$. Examples of $\augmentor{}$ include image cropping, or image-text pairing in CLIP. 
%T
%Typically,  $\Tilde{X} \in \Xc$ but it does not have to, \eg, in CLIP $A$ is a text but $X$ is an image.

\input{figures/schemas/losses/objectives}


%For notational convenience, we assume that we are optimizing over parameters of variational families, and that the encoder is deterministic $Z = e_{\theta}(X)$. For derivations see \toappx{}.


% \subsubsection{Exact}
% \label{sec:exact_issl}
%  \tofill{} This only works when you know $M(X)$ and is essentially what is happening when you do transfer learning while freezing a part of the network.


\subsection{Contrastive ISSL (CISSL)}\label{sec:contrastive_issl}

For the first method, we bypass the requirement of a maximal invariant by noticing that $\Mx{A}$ only appears as an index of a weight matrix $W$.
Without approximations, we can thus replace $W[\Mx{A}]$ by optimizing over any $g : \Xc \to \mathbb{R}^d$ which will learn to map example equivalent examples $x^+$ to corresponding weights, \ie, $g(x^+) = W[\Mx{A}(x^+)]$.
In practice $g$ will be parametrized, but we use $\inf_g$ to remind the reader that $g$ should theoretically be unconstrained.

The remaining challenge then becomes computing the normalizing constant without enumerating over classes. 
To do so we use the ranking conditional \cite{jozefowicz_exploring_2016,ma_noise_2018}  \textit{noise contrastive estimation} (NCE; \cite{gutmann_noise-contrastive_2010}).
NCE essentially replaces classification of the equivalence class by classifications of positives in a sequence $\mathbf{\view{}} \defeq \{ \view{}^+, \view{}^-_1, \dots, \view{}^-_k \}$ where the positive $\view{}^+$ is sampled from the conditional $\augmentor{}(\view{} \cond X)$, while negatives $\view{}^-_i$ come from the marginal $\augmentor{}(\view{}) = \Epmini{\p{X}}{\augmentor{}(\view{}|X)}$.
Using Monte Carlo (MC) estimates with dataset $\Dc$, we get the contrastive ISSL (CISSL) loss 
%
\begin{equation}\label{eq:cissl}
\Lc{}(\theta; \Dc) \defeq
\inf_{\phi \in \Phi,g} \sum_{x \in \mathcal{D}}
\Ep{
\augmentor{}(\mathbf{\view{}}|x)
}{
- \log \frac{\exp g(\view{}^+)^T h_{\phi}(Z_{\theta}(x))  }{\sum_{\view{}' \in \mathbf{\view{}} } \exp g(\view{}')^T h_{\phi}(Z_{\theta}(x))  }}.
\end{equation}
%

Ranking NCE is consistent and Fisher efficient \cite{ma_noise_2018}, meaning that as the number of negatives increases $|\mathbf{X}| \to \infty$, learning representations with the contrastive loss  $\argmin_{\theta}  \Lc{}(\theta; \Dc)$ is similar to direct ERM $\argmin_{\theta} \eRisk{\Mx{A}}{Z_{\theta}; \Dc}$ for the desired objective.


In standard cases where $\view{},X$ take value in the same space (\eg images),  we can tie parameters by encoding $\view{}$ before $g$, \ie, $g(Z_{\theta}(A))$. \ydnote{such parameter sharing does not change theoretical property if $g$ is unconstrained}
As an illustration, let us also suppose that downstream predictors $\Q$ are linear. %, so that $h_\theta(Z) = Z$ is the identity.
CISSL would then $\scores{}(\view{},z) = g(Z_{\theta}(\view{}))^T z$.
This is strikingly similar to SimCLR's InfoNCE objective \cite{chen_simple_2020}, which uses $\scores{}(\view{},z) = g(Z_\theta(\view{}))^T g(z)$ where $g$ is referred to as a projection head.
The only difference is that SimCLR projects the representations $z$ with $g$, thereby failing to ensure downstream linear predictability.
In contrast, CISSL formalizes the intuition that if task logits will be computed using $W^T z$ then SSL logits should be $W^T z$ instead of $W^T g(z)$.
%This also explains why improving the InfoNCE bound is detrimental for downstream tasks \cite{tschannen_mutual_2020}.
Entirely removing projection heads, \ie, $Z_\theta(\view{})^T z$, is also detrimental in practice \cite{chen_simple_2020}.
Indeed, this greatly constrains the mapping from $A$ to the desired weight matrix $W$.
CISSL instead derives from first principles the asymmetric use of projection heads. \footnote{
CLIP used asymmetric CISSL to deal with text $\view{}$ and images $X$. Projections were then undesirable.}
\ydnote{ drop footnote?  make it part of text ?}

The usefulness of CISSL goes beyond the typical (but unrealistic) assumption of linear predictors $\Q$.
E.g. CISSL can ensure discriminativeness to predictors with particular hidden architectures $h_{\phi}$ (\eg MLP or transformer) by computing logits as  $g(Z_{\theta}(\view{}))^T h_{\phi}(z)$. 
To our knowledge we are the first to show why a projection head is needed, why their current use is not sound, and how to perform contrastive learning for non-linear discriminativeness.
%For more discussion about how other experimental results can be understood  (such as 


\subsection{Distillating ISSL (DISSL) }\label{sec:distillation_issl}
\ydnote{This section is very dense and long. Thoughts on what to cut \percy{} ?}

% CISSL has the advantage of not estimating $\Mx{A}$ or fixing the number of equivalence classes, but it requires a large number of negatives $A^-$.
CISSL requires a large number of negatives $\view{}^-$ which can be prohibitive.
In this section we overcome the need for negatives by directly estimating $\Mx{A}$ using a categorical distribution $\teacher{}(\hMx{A} \cond x)$.
 Once we have an estimate $\hMx{A}$, we can learn $Z_\theta$ by minimizing the resulting $\Riskmini{\hMx{A}}{Z_{\theta}}$.
To highlight similarities with previous methods \cite{caron_unsupervised_2020,caron_emerging_2021,fang_seed_2021}, we refer to $\Riskmini{\hMx{A}}{Z_{\theta}}$ as \textit{distilling} the \textit{teacher} $\teacher{}(\hMx{A} \cond x)$ into a \textit{student} $\student{}(\hMx{A} \cond z)$ and the desired encoder $Z_\theta$. 
Replacing terms in  \cref{eq:obj_to_appx} we get 
%
\begin{equation}\label{eq:distillation}
\Risk{\hMx{A}}{Z_{\theta}} \defeq  \inf_{\phi \in \Phi, W} \Ep{t(\hMx{A} \cond X)\p{X}}{- \log \student(\hMx{A} \cond Z_{\theta}) }, 
\quad  s(m \cond z) \defeq \mathrm{softmax}(W^T h_{\phi}(z))[m]
\end{equation}
%$\Riskmini{\hMx{A}}{Z_{\theta}} \defeq \Epmini{t(\hMx{A} \cond X)p(X)}{- \log s(\hMx{A} \cond z)}$, where $s(m \cond z) = \mathrm{softmax}(W^T h_{\phi}(z))[m]$
%
The remaining challenge then becomes training  the teacher $t(\hMx{A} \cond x)$ to estimate $\Mx{A}$.
To do so, let us recall that by definition $\hMx{A}$ is desired a maximal invariant iff it is:
\begin{description}[noitemsep]
\item[Deterministic] the conditional entropy is $\mathrm{H}[\hMx{A} \cond x] = 0$;
\item[Invariant] mapping equivalent examples together $x \sima x^+ \implies t(\hMx{A} \cond x) = t(\hMx{A} \cond x^+)$; 
\item[Maximal] mapping non-equivalent examples separately $x \not\sima x^- \implies t(\hMx{A} \cond x) \neq t(\hMx{A} \cond x^-)$. 
\end{description}

Recent ISSL methods can be seen as various approximations of those %necessary and sufficient
requirements. 
%To our knowledge those requirement have never been formalized, but, 
In \cref{sec:appx:related} we provide a taxonomy of $>$30 objectives (\eg DINO \cite{caron_emerging_2021}, SwAV \cite{caron_unsupervised_2020}, MOCO \cite{he_momentum_2020}, SimSiam \cite{chen_exploring_2021}) from this perspective. 
Essentially, previous work favor
\begin{inlinelist}
\item determinism by ``sharpening'' the teacher $p(\hMx{A} \cond x)$;
\item invariance by forcing the teacher's and student's output to be similar for equivalent inputs $\teacher{}(\hMx{A} \cond x^+) \approx \student(\hMx{A} \cond x)$;
\item maximality through optimization tricks (\eg stop gradients or momentum teacher)
to avoid learning a constant teacher, \ie, referred to as ``collapsing'' \cite{chen_exploring_2021,ermolov_whitening_2021,he_momentum_2020,grill_bootstrap_2020}. 
\end{inlinelist}
\footnote{Avoiding constant collapsing is insufficient, \eg, mapping half the inputs to a constant is also undesirable.
Maximality formalizes the desired requirement: non-equivalent examples should not be mapped together.}

Given the formal requirements for the teacher we can derive a new approximate distillation ISSL (DISSL) method from first principles.
%For each requirement we use information theoretical quantities that can be computed in closed form for categorical distributions $\teacher{}(\hMx{A} \cond x^+)$ and 
%We use information theoretical quantities as those 
%We will use information theoretical quantities as th
First, let us consider the simpler invariance and maximality requirements.
For determinism we minimize the conditional entropy $\mathrm{H}[\hMx{A} \cond x]$.
For invariance we minimize the KL divergence of the teacher's output on equivalent inputs $\KLmini{\teacher{}(\hMx{A} \cond x)  }{\teacher{}(\hMx{A} \cond x^+)}$.
By expanding the KL divergence, we have that the teacher is invariant and deterministic iff the cross-entropy $\Epmini{\teacher{}(\hMx{A} \cond x)}{- \log \teacher{}(\hMx{A} \cond x^+) }$ is minimized to 0.

Let us now consider maximality.
We could enforce it by assuming access to many negatives $x^- \not\sima x$, but this is CISSL's weakness that we aimed to avoid.
Instead, we assume that we know (or have a prior on) the marginal of the equivalence classes $p(\Mx{A})$.
If the teacher is invariant and deterministic, we can then enforce its maximality by minimizing the KL divergence between  the teacher's marginal $\teacher(\hMx{A}) = \Epmini{\p{X}}{\teacher(\hMx{A} | X)}$ and the true one, \ie, $\KLmini{\teacher{}(\hMx{A})  }{ p(\Mx{A})}$.
Importantly, 
%if a conditional distribution $\teacher(\hMx{A} | X)$ is categorical then so is the marginal $\teacher(\hMx{A})$.
the marginalization and KL can be efficiently computed in closed form for categorical distributions.
Putting altogether with \cref{eq:distillation}, using Lagrangian 
multipliers $\lambda,\beta$, MC estimates,
and denoting $\mathbf{\view{}} = \{\view{},\view{}^+\}$ as two samples from the augmentor $\augmentor{}$,
we get the DISSL loss $\Ld{}(\theta; \Dc) \defeq$
%
\begin{equation}\label{eq:dissl}
\inf_{\phi \in \Phi,W,t} \sum_{x \in \mathcal{D}}
\lambda \KL{\teacher(\hMx{A}) , p(\hMx{A})} 
- \Ep{
\augmentor{}(\mathbf{\view{}}|x) \teacher{}(\hMx{A} \cond \view{})
}{
\log \student{}(\hMx{A} \cond Z_{\theta}(x)) 
+ \beta \log \teacher{}(\hMx{A} \cond \view{}^+) 
}.
\end{equation}
%
%where, as with CISSL, the infimum makes it clear that the teacher should be unconstrained but the logits of the student should take the form of the desired downstream predictors $W^T h_{\phi}(z)$.
DISSL is essentially equivalent to the desired $\Risk{\Mx{A}}{Z_{\theta}}$ when the marginal $p(\Mx{A})$ is known.
When it is unknown, we will,  by the max entropy principle \cite{jaynes_information_1957}, assume that it is a uniform over some selected number of equivalence classes $p(\Mx{A}) \approx \mathrm{Unif}(1,\hcalMx{A})$.
%Typically, we will use a uniform prior $p(\Mx{A})$, in which case $\min \operatorname{D}_{\text{KL}}$ turns into maximization of the marginal entropy $\mathrm{H}[\hMx{A}]$.

\input{figures/algorithms/DISSL_wrap}
As with CISSL, when $\view{},X$ are in the same space, we tie parameters by encoding $\view{}$ before the teacher, \ie, $\teacher{}(\hMx{A} \cond Z_\theta(\view{}))$.
\Cref{alg:DISSL} shows the resulting algorithm when predictors $\Q$ are linear, the prior is uniform, and the marginal is computed from batches (not required, see \cref{sec:appx:deriv:cissl}).
DISSL is then very related to previous methods such as DINO and SwAV.
The main differences being that DISSL enforces maximality in a simpler way (no gradient stopping, momentum teacher, queue, or Sinkhorn-Knopp algorithm \cite{sinkhorn_concerning_1967}) and ensures linear predictability by avoiding projection heads.
%Indeed, previous methods fail to ensure linear predictability as they use projection heads like in SimCLR.
Details in \cref{sec:appx:deriv:cissl}.

\subsection{Generative ISSL (GISSL) }\label{sec:generative_issl}

\ydnote{Should we removed generative from the main text and put it to appcs, \percy{} ? 

The two reasons I see for keeping it is:
(1) shows that the theoretical framework is very general as we can analyse all previous classes of methods; 

(2) have the experiments showing that we significantly improve generative models (although there are still bad)


But it does read more like an afterthough for now, and I don't want to spend much space on that. 
}

Another typical way of learning representations $Z$ is with generative models \cite{liu_self-supervised_2021} that aim at learning a $Z$ that allows reconstructing or generating inputs
\cite{kingma_auto-encoding_2014,vincent_extracting_2008,donahue_adversarial_2017,radford_unsupervised_2016,dumoulin_adversarially_2017}
%, \eg variational autoencoders (VAE;  \cite{kingma_auto-encoding_2014}), denoising AE (DAE; \cite{vincent_extracting_2008}), or adversarial methods \cite{donahue_adversarial_2017,radford_unsupervised_2016,dumoulin_adversarially_2017}. 
Although generative ISSL is very successful in natural language processing (NLP) \cite{brown_language_2020}, it is not competitive in vision. %\cite{liu_self-supervised_2021}
We see at least two potential reasons.
First, those methods rarely incorporate data augmentations and thus use the worst (finest) equivalence structure given by the identity.
Second, generative models do not ensure linearly discriminativeness as they use complex non linear mapping from representations to reconstructions. In \cref{sec:appx:deriv:gissl} we propose a generative ISSL (GISSL) objective that solves those issue.
The intuition, illustrated in \tocref{}, is to encode augmented inputs $\view{}$ into the representation $Z$ and then reconstruct unaugmented inputs $X$ using a decoder that ensures linear discriminativeness.










==> text/background.tex <==
\ydimp{
I removed the figures on M(X) as suggested by \tatsu{}. So now it's very short. Should we merge this to section 4 (either subsection or first para of 4.1)?
}

The key for our theory, is that there always exists a function $M(\cdot)$, called the maximal invariant, such that any function invariant to $\sim$ can be written as a function of $M$ \cite{dubois_lossy_2021}.
The maximal invariant $M(\cdot)$, is any function that essentially indexes the equivalence class,
%
\begin{equation}\label{eq:Mx}
x \sim x^+ \iff M(x)   = M(x^+) \quad \forall x,x^+ \in \Xc.
\end{equation}

%\input{figures/schemas/Mx/wrap_Mx}

% 
%In other words, $M(X)$ is a minimal sufficient statistic that retains all and only the information invariant to $\sim$.
%For data augmentations, the unaugmented inputs is a maximal invariant. %See \cref{fig:max_inv}.
%\cite{mac_lane_algebra_1999,dubois_lossy_2021}. 

% Finally, two useful concepts in equivalence relations are \textit{refinements} and \textit{coarsening}.
% To illustrate them, consider the modulo 10 equivalence relation $\sim_{10}$ on natural numbers, \ie, equivalence classes are given by the last digit of a number.
% Then modulo 100 arithmetic $\sim_{100}$ would give a \textit{refinement} of $\sim_{10}$, because numbers that have the same last 2 digits must also have the same digit.
% Formally, $\sim_r$ is a refinement of $\sim$, denoted $\sim_r \subseteqs \sim$, iff for every equivalence class of the former $[x]_r \in \mathcal{X}/\sim_r $ there is an $[x] \in \mathcal{X}/\sim $ s.t. $[x]_r \subseteq [x]$.
% Analogously, we say that $\sim_{10}$ is a \textit{coarsening} of $\sim_{100}$.
% Note that any function $f$ that is invariant to some equivalence $\sim$ will be invariant to any refinement $\sim_r$.
% For example, MNIST labels are trivially invariant to the equivalence defined by the labels, but also to any refinement such as the one shown in \cref{fig:Mx_augmentation} that partitions different ``7'' into distinct classes.



% \ydnote{Need to add about refinement and coarsening, specifically, that if you have a refined equivalence relation then you also have all information you need about the coarser one}

==> text/decodability.tex <==
\input{figures/schemas/geometry/geometry}

 For a representation to be discriminative it essentially needs to have information about all downstream tasks $\tasksinv{}$ in a way that is extractable by $\Q$.
To build intuition about when that happens, consider 
%We will prove that this happens if and only if one can predict a maximal invariant $M(X)$ from $Z$ using the correct functional family $\Q$, under some shatterability constraint. %a constraint that any binary labeling of the equivalence classes can also be predicted.
an equivalence $\sim$ partitioning $\Xc$ into 4 classes: cats, dogs, oranges, and lemons.
Then $\tasksinv{}$ consists of all tasks predictable from the equivalence class, \eg, animals vs fruits $Y_{\scriptscriptstyle \mathrm{A;F}}$, or oranges vs rest $Y_{\scriptscriptstyle \mathrm{O;R}}$.
In other words, downstream Bayes predictors are invariant to $\sim$ and can thus be written as functions $g$ of a maximal invariant, \ie, $\argmax_{y} p(y|X) = g ( M(X))$.


When predictors are unconstrained $\U$, if there is a function $f$ from representations to maximal invariants $f(Z)=M(X)$ then one can perfectly predict downstream tasks with $\argmax_{y} p(y|X) = g(f(Z))$ because $g \circ f \in \U$.
\Cref{fig:geometry_zu} shows such a representation, but not \cref{fig:geometry_zb}

For constrained functional family $\Q$, \eg, linear predictors,  we could think that we only need linear seprability of the equivalence classes, \ie, $f \in \Q$ s.t. $f(Z)=M(X)$.
This is nevertheless not sufficient because the composed $g \circ f$ might not be linear anymore.
For example, \cref{fig:geometry_zl} provides linear separability of $M(X)$, but not for animal/fruit $\rv Y_{\scriptscriptstyle \mathrm{A;F}} \in \tasksinv$ as shown in \cref{fig:geometry_zns}.

Intuitively, a good representations should thus not only minimize $\Risk{M(X)}{Z}$ but also ensure that any relabeling should be separable by $\Q$ (as in \cref{fig:geometry_zs}).
Specifically, we need any binary labeling of the equivalence classes to also be predictable.
We call such constraint ``$\sim$-shattering'' of the encoder.
%We prove the intuition in \cref{sec:appx:proofs:disc}, which can be formalised as follows.
%
\begin{definition}
An encoder $\p{Z|X}$ is \textit{$\sim$-shattered by $\Q$} iff any binary labeling $b : \Mc \to 2$ of equivalence classes can be predicted by an $f \in \Q$, \ie, $f(Z) = b(M(X))$.
We denote those encoders as $\sP{}$.
\end{definition}

\begin{theorem}\label{thm:main}
An encoder $\p{Z|X}$ is discriminative for $\tasksinv{},\Q$ if and only if $\p{Z|X}$ minimizes $\Risk{M(X)}{\rv Z}$ and  it is $\sim$-shattered by $\Q$, \ie,
\begin{equation}\label{eq:optimal}
\argmin_{\p{Z|X}} \distsA{} = \argmin_{\p{Z|X} \in \sP{}  } \RiskA{M(X)}{\rv Z}.
\end{equation}
\end{theorem}

\ydnote{
Not sure if worth saying but we actually have $\distsA{}=0$ which means that replacing the sup with an expectation over tasks would give the same result.
}

%Furthermore, for discriminative encoders we have $\distsA{}=0$. 
\Cref{thm:main} shows that instead of performing all infinite invariant tasks $\tasksinv{}$ of interest, we can learn the desired representations by performing a \textit{single} pretext task under a decodability constraint.
This pretext task consists of predicting the equivalence class or recognizing equivalent examples from the representation  using the correct predictors $\Q$.
Importantly, when the encoder is unconstrained both sides of \cref{eq:optimal} (the pretext task and the worst-case excess risk) can achieve the minima 0. %, $\min_{\p{Z|X} \in \sP{}  } \RiskA{M(X)}{\rv Z}=0$, so we can estimate how far we are from optimality.
%Importantly, $\sim$-shattering 
%Importantly, one has to perform ISSL ISSL with respect 

%This is possible because we know the underlying invariance structure $\sim$ and the downstream predictive family $\Q$.

% In practice we do not have access to the maximal invariant, but we have access to samples from $\rv X$ and random transformations of it $\A \dsim \p{\A|X}$ that give the equivalence structure $\sim$.
% In this case we prove in \tocref{} that we can then essentially replace $\Q$ classification of $M(X)$ by $\Q$ predictability of the augmented source $A$.


%This shows the power of (I)SSL, by having partial know
%The relation between the worst case risk and the pretext task is actually even deeper. 
%Indeed, \tocite{} have shown that when the evaluation loss $L$ is the log loss and $\Q$ is unconstrained then $\Risklog{M(X)}{\rv Z}$ is exactly equal to the worst excess risk \cref{eq:worst_case} for all encoders (not only the optima).

%Furthermore, we show in \toappx{} that the pretext task $M(X)$ is minimal in the sense that it retains no additional information about the input $\rv X$.
%We also prove that considering invariants tasks $\tasksinv{}$ is necessary and sufficient for the existence of a minimal pretext task.

% As \cref{thm:main} is an if and only if statement, it shows that maximal invariants $M(X)$ with shatterability w.r.t $\sim$ are essentially minimal sufficient pretext tasks for ISSL.
% There are nevertheless many other sufficient pretext tasks, specifically, any maximal invariant $\Mx{r}$ of a refined equivalence $\sim_r \subseteq \sim$.

%This is true in the case where encoders are shatterable w.r.t  $\sim$ or to $\sim_r$, but the latter is more constrained.

% \begin{proposition}\label{prop:sufficient_refine}
% Let $\tasksinv{},M,\Q$ be as in \cref{thm:main}. 
% Let $\sim_r \subseteq \sim$ be a refinement of the desired equivalence  with maximal invariant $\Mx{r}$.
% Let $\oP{\sim}{M} \defeq \argmin_{p(Z|X) \in \sP{}  } \RiskA{M(X)}{\rv Z}$ denote the encoders that can predict $M$ and are shattered w.r.t $(\mathcal{X},\sim)$.
% We have:
% \begin{equation} \label{eq:sufficient_refine}
% \oP{\sim_r}{\Mx{r}} \subseteq \oP{\sim}{\Mx{r}}  \subseteq \oP{\sim}{M}.
% \end{equation}
% \end{proposition}
% %

% \Cref{prop:sufficient_refine} shows that predicting $\Mx{r}$ with shattering w.r.t. $\sim_r$ or $\sim$ is a sufficient pretext task.
% Indeed, resulting encoders are subsets of $\oP{\sim}{M}$, so by \cref{thm:main} they minimize the desired excess risk $\distsA{}$.
% As illustration, suppose $\Q$ is linear and the desired $\sim$ consists in 2 equivalence classes: cats-dog vs orange-lemon.
% Then examples of encoders for each sets in \cref{eq:sufficient_refine} would be:
% \cref{fig:aug_mx} for $\oP{\sim}{M}$; 
% \cref{fig:aug_A} for $\oP{\sim}{\Mx{r}}$;
% \cref{fig:geometry_zs} for $\oP{\sim_r}{\Mx{r}}$.

==> text/implications_old.tex <==
We will now take advantage of the if and only if in \cref{thm:main},
to derive practical insights into ISSL. 




\subsection{Sample efficiency}
\label{sec:sample_efficiency}
\input{text/sample}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{What dimensionality of $Z$ to use ?}
\label{sec:dimensionality}

% \Cref{thm:main} says that optimal representations should allow separability of $M(X)$ and shattering by $\Q$.
% We now show that these requirements directly impact the choice of $\Zc$.

%\paragraph{Dimensionality}
%What is the required dimensionality $d_{\Q}$ of $\mathcal{Z}$ for an encoder to satisfy \cref{thm:main}?
Due to the shattering requirement, there is a necessary and sufficient representation's dimensionality $d_{\Q}$ for an encoder to satisfy \cref{thm:main}.
For example, in \cref{fig:geometry_zs} we provided a representation that can be shattered by increasing  dimensions to $d=3$ compared to $d=2$ in \cref{fig:geometry_zl}.
Increasing $d$ is necessary. 
%; a 2D representation cannot be linearly shattered for four equivalence classes.
Indeed, linear predictors $\Q$ can only shatter up to $d+1$ points. 
As a reminder, the maximal points that can be shattered by $\Q$ is the \textit{VC dimension} of $\Q$ \cite{vapnik_uniform_1971}.
%
\begin{proposition}\label{prop:VC_dimension}
There exists an encoder $\p{Z|X}$ that is $\sim$-shattered by $\Q$ if and only if the VC dimension of $\Q$ is at least the number of equivalence classes, \ie,  $\mathrm{VC}(\Q) \geq \nequiv{}$.
\end{proposition}
%
%VC dimensions is often used in bounds, but here \cref{prop:VC_dimension} provides an exact results. 
%By taking advantage of established results in VC dimension \tocite{} we can also give tight estimates of the desired dimensionality $d_{\Q}$ for $\Q$.
%Furthermore, we can take advantage of well known results in VC dimensions \tocite{}.
%
%We can use standard VC dimension results \cite{shalev-shwartz_understanding_2014} to characterize the dimension $d_{\Q}$ for different $\Q$.
%
\begin{corollary}\label{cor:dimension}
From standard VC dimension results \cite{shalev-shwartz_understanding_2014}, the minimal and sufficient dimension $d_{\Q}$
\begin{multicols}{2}
    \begin{itemize}
    \nolinenumbers
        \item is $d_{\Q_l} = \nequiv{} - 1$ for linear predictors $\Q_l$;
        \item increases for any $\Q^- \subseteq \Q$, \ie,  $  d_{\Q^-} \geq d_{\Q}$;
        \item decreases with parameters in MLPs;
        \item is $d_{\U} = 1$ for unconstrained predictors $\U$.
    \end{itemize}
    \end{multicols}
\end{corollary}
%
% \ydnote{despite trying my best otherwise right now I'm worried that the general DL public will find the paper to theoretical too parse. But in reality I think that what we are saying is quite intuitive. 

% These prescriptive summaries (and the ones below) at the end of every subsection is one way of trying to alleviate this issue, but likely not sufficient. 
% }
In summary, the shattering requirement gives a tight required dimensionality of $Z$, which is at most the the number of equivalence classes and decreases for more complex $\Q$.% for predictors that are at least linear.
%In practice, it may not be recommended to use larger $d$ due to computational and sample efficiency issues.
%of course the (effective) dimensionality should not be arbitrarily large.
%This is best seen from the lens of generalization, as larger $d$ often increase the Rademacher complexity of $\Q$ which means that more downstream samples could be needed for generalization \tocref{}.
%In practice, larger $d$ also make learning less computationally efficient.

% \paragraph{Cardinality of the sample space $|\mathcal{Z}|$}
% For a representation to minimize $\RiskA{M(X)}{Z}$ there needs to be at least one point per equivalence class, \ie, $|\mathcal{Z}| = |\mathcal{X} / \sim |$ to avoid mapping different equivalence classes to the same encoder.
%This is typically already satisfied.
%\ydnote{This seems trivial, but could be important in the case where you use discrete Z like VQVAE ?}

%Indeed, if that was not true then two equivalent classes would have to be mapped to the same representation by the encoder.

\subsection{What augmentations to use during ISSL ?}
\label{sec:augmentation}

In ISSL practitioners incorporate information about downstream tasks through invariances by sampling equivalent example, \eg, using data augmentations.
But this information is only partial, \ie, although classification tasks will be invariant to standard augmentations $\sima$ we only care about a subset of such tasks , \ie,  $\tasksinv{} \subseteq \tasksinva{}$.
Formally, the practitioner only has access to an equivalence  $\sima$ that is \textit{finer} than the equivalence structure $\sim$ of desired tasks, \ie, $x \sima x^+ \implies x \sim x^+$.
%In other words, the equivalence structure $\sim$ of desired tasks is \textit{coarser} than the practioner's one $\sima$.
%\ydnote{repeating to introduce people to these notions, not sure if necessary.}
Such finer $\sima$ is nevertheless sufficient to learning discriminative encoders for the desired $\tasksinv{}$.
%
\begin{proposition}\label{prop:sufficient_refine}
Let $\sima$ be an equivalence that is finer than $\sim$.
Then any encoder $\p{Z|X}$ that is discriminative for $\Q,\tasksinva{}$ is also discriminative for $\Q,\tasksinv{}$
\begin{equation}
\argmin_{\p{Z|X} \in \sPa{}  } \RiskA{\Mx{A}(X)}{\rv Z}
\subseteq 
\argmin_{\p{Z|X} \in \sP{}  } \RiskA{M(X)}{\rv Z} 
\end{equation}
\end{proposition}
%
\Cref{prop:sufficient_refine} shows that one does not require access to unrealistic augmentations to learn discriminative encoders. 
This contrasts with most previous theoretical work in SSL that assume unrealistic conditional independence $\A \indep X \cond \tasks{}$ \cite{saunshi_theoretical_2019,lee_predicting_2020,tosh_contrastive_2021} --- a notable exception being \cite{haochen_provable_2021}.
In particular, we have that any label-preserving augmentor $\augmentor(\view | X)$ s.t. $\view \sima X$  are sufficient.
This is surprising as it means that even the identity $\view{} = X$ is sufficient. 
Yet such augmentations clearly seems less useful.

The reason is that, out of the equivalence that are finer than $\sim$, coarser ones are better in three aspects: 
(Dimensionality)  \cref{cor:dimension} shows that required dimensionality increases with $\nequiva{}$ ;
(Sample efficiency)
\cref{sec:sample_efficiency} shows that the number of required downstream samples scales at best linearly with $\nequiva{}$;
(Optimization) \cref{prop:sufficient_refine} shows that the number of discriminative encoders is smaller for finer equivalences, suggesting that optimization will be harder.

%\ydnote{Can dropt this paragraph if need space}
%As an illustration achieving the Bayes risk on tasks $\tasksinv{}$ using the identity augmentation $\A=X$ and linear predictors $\Q$  would require:
%\begin{inlinelist}
%\item a representations of dimension $|\Xc|-1$;
%\item seeing every example once in downstream datasets; and
%\item solving a hard optimization problem.
%\end{inlinelist}
%These requirements are unrealistic, which aligns with the intuition that the identity $\A$ (finest equivalence) is not useful.

In summary, any label preserving augmentation is sufficient for learning discriminative encoders, but those that give coarser $\sim_A$ are more useful.
Examples of coarse ISSL are methods that use multi-modal data 
\cite{alayrac_self-supervised_2020,wang_multimodal_2021,akbari_vatt_2021}, \eg, CLIP 
\cite{radford_learning_2021} which maps many equivalent images to similar sentences.
\ydnote{should look for previous literature, if there are other papers that prove or suggest the advantages of coarse augmentations they should be cited here
}
\ydnote{
can give as example the fact that CLIP uses 4x smaller dimensions}
%In practice, such methods indeed provide and require smaller representations dimensionality.


\subsection{What family $\Q$ to use during during ISSL ?}
\label{sec:predictive_family}

\Cref{thm:main} shows that to learn discriminative encoders one has to ensure predictability of $M(X)$ and $\sim$-shatterability for the actual predictors $\Q$.
This nevertheless does not mean that we have to learn an encoder for every possible predictive family $\Q$, which would be computationally intensive.
Indeed, ensuring discriminativeness for smaller predictors $\Q^-$ implies it for a larger $\Q^+$.
%
\begin{proposition}\label{prop:predictive_family}
Let $\Qm,\Q$ be families s.t. $\Qm \subseteq \Q$. 
Any encoder $\p{Z|X}$  that is discriminative for $\tasksinv{},\Qm$ is also discriminative for $\tasksinv{},\Q$.
\end{proposition}
%
\Cref{prop:predictive_family} shows that performing ISSL with respect to a smaller family $\Qm$ (\eg linear) than the actual predictors $Q$ (\eg MLP) is sufficient. 
In practice, this will nevertheless make optimization harder (less encoders are $\Qm$ discriminative) and increase the required dimension by \cref{prop:VC_dimension}.
%Importantly, the converse is not true so it i


% \subsection{What regularization to use ?}
% \label{sec:improve_sample}

% \ydimp{weak section to rewrite once decided what to say}

% In \cref{sec:sample_efficiency} we have shown that we can achieve sample efficient encoders by learning invariant encoders. 
% In practice, this suggests using regularizers that ensure $\supp{\p{Z|x}} = \supp{\p{Z|x^+}}$ for equivalent  $x\sim x^+$, \ie, regularizers that favor collapsing representations from equivalent examples.

% Explicitly this can be done in many ways, some of which essentially already appeared in the literature \cite{wang_deep_2017,sinha_consistency_2021,dubois_lossy_2021,ruan_optimal_2021,federici_information-theoretic_2021,lee_compressive_2021,mitrovic_representation_2021,tomasev_pushing_2022}
% , \eg, by minimizing any of $\KL{p(Z|X), p(Z|\A)}$, $\MI{Z}{X | M(X)}$, $\MI{Z}{X}$ or $\H{Z}$.
% The choice of regularizer should then depend on practical optimization, but our theory provides many new regularizers to consider.
% In our experiments we consider a regularizer $\Ep{}{\|e(X) - e(A)\|}$ that is easier to estimate but still ensures sample efficiency for deterministic encoders $e$.


% Interestingly many previous papers have suggested (empirically and theoretically) that neural networks trained with SGD actually push towards $\supp{\p{Z|x}} = \supp{\p{Z|x'}}$ once the training loss essentially reaches the Bayes optima \tocite{}.
% I.e. when training long enough with overparametrized networks and enough stochasticity, the inter equivalence variance essentially decreases. 
% Our theory thus gives more insight into why long training, and overparametrization is desirable and close to optimal.




% First, we see that encoders from \cref{thm:main} are not equally good in practice, and that invariant support implies better sample efficiency.
% As a result, we can add different regularizers to ensure better sample efficiency, \eg, if we are using label-preserving augmentations ($\A \sim X$) then we can regularize $\KL{p(Z|X), p(Z|\A)}$. 
% Improving sample efficiency can also be achieved by other regularizers, \eg, by $\MI{Z}{X | M(X)}$, $\MI{Z}{X}$, or $\H{Z}$.
% \ydnote{
% I thought that what would be needed is DIB but that might not be the case because you still want shaterability in which case I think minimizing $I_V[Z,X]$ might just be $I[Z,X]$. 
% For next paper it might worth trying to analyze the IFF of that statement.
% }



% \ydnote{
% Actually the equivalence class that you need is probably given by which X mapped to you. I.e. not by connected component but actual neighboorhood or something.
% Because essentially you want Z to have the same support for all x in the connected component.
% As long as this is done then you only need one example.
% And note that this is possible if you have connected component augmentation and use $p(Z|\Tilde{X})=p(Z|X)$ for all augmentations.
% Although all of that really just shows that what you want is $R[M(X)|Z]$ under shattering constraint and min $I[Z,X]$ which is possible by minimizing $R[M(X)|Z]$ and $KL[p(Z|X),p(Z|\Tilde{X})]$ and shattering if the augmentation graph has a connected component that covers the equivalence class.
% }
%In practice this means trying to use augmentations that remove more information about ``which source example you came from ''

%In practice using $A(X) \indep X \cond M(X)$ is very unrealistic.We will now show that the same advantages can be achieved using realistic augmentations (where the connected components of the augmentation graph cover the desired equivalence class) by changing the loss that is used in ISSL, specifically by adding one additional constraint, \ie, $p(Z|x) = p(Z|A(x))$ for all $x \in \mathcal{X}$.
%Indeed, in that case
%\ydnote{
%It's not actually equivalent because $\Risk{M(X)}{Z}$ will nto necessarily recover something like $Z=M(X)$.
%But when using the regularizer you can show that both are equivalent and are essentially the optima.
%}



% \subsection{Choosing the predictive family $\Q$}
% \label{sec:predictive_family}

% \ydnote{I don't really know what to make our of that section. It kind of seems trivial.  thoughts ?

% also I was planning on discussing what the downstream predictors should be. I.e. but I don't think there' much to add there}

% Until now we assumed that predictors $\Q{}$ were fixed and known.
% In reality, $\Q$ is also a variable to select and might change depending on the downstream user.
% This adds an additional question, namely, w.r.t. to what family should the representation be learned ?
% Here we show that representations should essentially be trained w.r.t. to small $\Q$.

% We have seen in \cref{thm:main} that representations should minimizes $\RiskA{Y}{Z}$ and be shaterable w.r.t to the desired $\Q$.
% It is nevertheless easy to show that satisfying these properties for smaller families $\Qm \subseteq \Q$ is sufficient.
% %
% \begin{proposition}\label{prop:smaller_Q_is_better}
% Let $\Qm,\Q$ be families s.t. $\Qm \subset \Q$. 
% Any $p(Z|X)$ satisfying \cref{thm:main} for $\Qm$ also satisfies it for $\Q$.
% \end{proposition}
% %
% In practice, the learned ISSL representation might be used with a variety of different downstream $\Q$, in which case \cref{prop:smaller_Q_is_better} suggests learning encoders w.r.t. to the smallest of those possible $\Q$, which is typically linear.

% Learning representations w.r.t. smaller families $\Qm{}$ does come at the cost of more complex representation learning stage. Indeed, encoders that are optimal for $\Qm$
% \begin{inlinelist}
% \item require a larger dimension of $\repspace{}$;
% \item are only a subset of those that are optimal for $\Q$ (\cref{prop:smaller_Q_is_better}).
% \end{inlinelist}
% Learning representations w.r.t. to smaller predictive families thus requires larger encoder families (so typically more data to train).
% Importantly, making the representation stage harder is nearly always beneficial compared to doing so for the prediction stage, because the work and computation is then amortized over all downstream use of the pretrained encoder.
% \ydnote{extremely informal, is it ok?}

%\paragraph{Use small downstream predictive families}

% \ydnote{We could probably add a quick discussion about what choice the downstream users should make for $\Q$.
% But that would essentially say the same as here: smaller is better cause you amortize.
% + it would add that better generalization as they usually have less data.
% It is sort of trivial and not directly about rep learning, which is why I'm skiping. But maybe worth mentioning.
% }

% \subsection{Going beyond accuracy}
% \label{sec:beyond}

% Until now we have only discussed about the accuracy loss. 
% But \cref{thm:main} and other results can be generalized to common losses in ML such as log loss, MSE, MAE, \dots 
% Specifically, we can work with any losses (and associated tasks)
% \ydnote{actually it's not only an assumption on the loss but also an assumption on the task, which is why I have the parentesis}
% that are strictly proper \tocite{}
% \ydnote{This is a generalization of strictly proper scoring rules}, which ensures the existence of a unique Bayes predictor \tocite{}.
% Specifically, let $\ell : \labspace{} \times \actspace{} \to \mathbb{R}_{\scriptstyle \geq 0}$ be a loss function. We assume that for all $x \in \mathcal{X}$, there exist $\act^* \in \actspace$, such that for any other $\act \in \actspace$ we have $\Ep{\p{Y|x}}{\ell(Y, \act^*)} <\Ep{\p{Y|x}}{\ell(Y, \act)}$.
% \ydnote{
% It actually also puts some minor assumption on the marginal, but really minor so probably good for appcs.
% }

% Then we prove in \toappx{} that our \cref{thm:main} generalizes to any invariant task that preserves the Bayes predictor. 
% Specifically, let $\ell$ be a strictly proper loss and $\tasksinvL{}$ be the set of tasks $\rv Y$ that preserve the Bayes predictor, \ie, $x \sim x^+ \implies \bayes{Y|X}(x) = \bayes{Y|X}(x^+)$.
% For log loss this means invariance of conditional distribution, while for MSE it means invariance of the conditional mean.
% Then under suitable assumptions on $\Q$ we can show that:
% \ydnote{I think the assumptions equations might be nasty to explain here which is why I'm not writing all the paper with those.

% But supposing that they are not nasty should we ? what if there are indeed nasty ? \stefano{}
% }
% \ydnote{Need to add a constraint to ensure that you can predict any composition of functions. Have to think carefully about that.}

% \begin{equation}\label{eq:general_losses}
% \argmin_{p(Z|X)} \dists{} = \argmin_{p(Z|X) \in \sP{}  } \RiskA{M(X)}{\rv Z}  
% \end{equation}
%
% This shows that although not typical, ISSL can also be used to perform any task evaluated with a different loss. 
% Surprisingly, the right of \cref{eq:general_losses} is actually w.r.t. accuracy even if the left is not.
% So the choice of downstream loss does not impact the representation learning procedure.
% More generally we can prove that to perform ISSL w.r.t. to any strictly proper loss $\ell$ one needs to minimize $\RiskL{M(X)}{\rv Z}{\ell'}$ w.r.t. to any loss $\ell'$ that is information preserving \cite{dubois_lossy_2021}. 
%, \ie, s.t. $\RiskL{M(X)}{X}{\ell'} = \RiskL{t(X)}{Z}{\ell'}$ implies that there exists an $h$ s.t. $M(X) \aseq h(Z)$.
% Which is also the case for typical losses such as MSE, accuracy, log loss.
% \ydnote{
% This is a little of a mess, although the most general, maybe we should simply decide on one of those assumptions (the most stringent) and then say for any $\ell,\ell'$ we have $\argmin_{p(Z|X)} \dists{} = \argmin_{p(Z|X) \in \sP{}  } \Risk{M(X)}{\rv Z}{\ell'}$
% }


%Importantly the loss that is used for the $\Risk{M(X)}{\rv Z}$ does not actually need to be the same loss as $\ell$. 
% \ydnote{It can be any loss that is information preserving, but need to double check for augmentations, whether any information preserving loss is also sufficient. Because $A(X)$ is not deterministic any more.
% }


%\paragraph{Effect of loss $\ell$}

%\paragraph{Effect of functional family}

%\paragraph{Negative samples}

%\paragraph{Positive samples}

%\paragraph{Tightening the bound}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Why InfoMax is not desirable?}
% \label{sec:infomax}



% \subsection{Does SSL pull together positives?}
% \label{sec:positives}


==> text/introduction_old.tex <==


% \begin{table}
% \begin{center}
% \begin{small}
% \begin{tabular}{llrr}
% \toprule
% &&  Linear &  MLP   \\
% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Distil.  }}  
% & SimSiam & $40.1$ {\tiny $\pm 0.3$}   & $45.0$ {\tiny $\pm 0.3$} \\
% & SwAV & $40.3$ {\tiny $\pm 0.2 $}   & $ 40.7 $ {\tiny $\pm 0.1 $} \\
% & DINO & $43.1$ {\tiny $\pm 0.3$}  & $44.0$ {\tiny $\pm 0.4$} \\
% \cmidrule{2-4}
% & \textbf{DISSL}  {\tiny (ours)}  & $\mathbf{44.9}$ {\tiny $\pm 0.1$} & $\mathbf{45.6}$ {\tiny $\pm 0.2$} \\
% & \ + dim $\uparrow$   & $\mathbf{47.0}$  {\tiny $\pm 0.1$} &     \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}


% \begin{table}
% \caption{Linear probing, ImageNet, RN50, Acc.}
% \begin{center}
% \begin{small}
% \begin{tabular}{llr}
% \toprule
% &  &  100 ep.    \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Distl.  }}  
% & SwAV & $46.1$ \\
% \cmidrule{2-3}
% & \textbf{DISSL}  {\tiny (ours)}  & $\mathbf{46.9}$   \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}
% \caption{Linear probing, TinyImageNet, 500 epochs, RN18, Acc.}
% \begin{center}
% \begin{small}
% \begin{tabular}{llrr}
% \toprule
% &&  All &  5-shot   \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Cntr.  }}  
% & SimCLR & $44.6$ {\tiny $\pm 0.3$} & $16.6$ {\tiny $\pm 0.1$} \\
% \cmidrule{2-4}
% & \textbf{CISSL}  {\tiny (ours)}  & $\mathbf{45.3}$ {\tiny $\pm 0.2$} & $\mathbf{17.5}$ {\tiny $\pm 0.0$}   \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}
% \begin{center}
% \begin{small}
% \begin{tabular}{llrr}
% \toprule
% &&  All &  5-shot   \\
% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Cntr.  }}  
% & SimCLR & $44.6$ {\tiny $\pm 0.3$} & $16.6$ {\tiny $\pm 0.1$} \\
% \cmidrule{2-4}
% & \textbf{CISSL}  {\tiny (ours)}  & $45.3$ {\tiny $\pm 0.2$} & $17.5$ {\tiny $\pm 0.0$} \\
% & \ + dim $\uparrow$   & $\mathbf{51.3}$  {\tiny $\pm 0.1$}  & $\mathbf{18.4}$ {\tiny $\pm 0.2$}   \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}
% \begin{center}
% \begin{small}
% \begin{tabular}{llrr}
% \toprule
% &&  Linear &  MLP   \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\footnotesize  \centering ~Cntr.  }}  
% & SimCLR & $44.6$ {\tiny $\pm 0.3$} & $46.3$ {\tiny $\pm 0.1$} \\
% \cmidrule{2-4}
% & \textbf{CISSL}  {\tiny (ours)}  & $\mathbf{45.3}$ {\tiny $\pm 0.2$} & $\mathbf{46.8}$ {\tiny $\pm 0.2$} \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

Learning effective representations from large amounts of data with little human supervision is a long-standing problem \cite{hinton_learning_1986,hinton_unsupervised_1999,bengio_representation_2014,lecun_deep_2015}.
Recently, there has been many such breakthroughs \cite{jing_self-supervised_2019,jaiswal_survey_2021,chen_simple_2020,radford_learning_2021} using invariant self-supervised learning (ISSL), whereby humans provide partial supervision through objectives and augmentations that retain desired information. 
Despite empirical successes, it is unclear \textit{why} current ISSL methods work and \textit{how} to improve them.
Ideally, those questions would be answered using a theoretical and conceptual framework to analyze, derive, and compare any ISSL method.
\ydnote{This sentence should be much more convincing}

Despite important advances in (I)SSL theory \cite{tian_understanding_2021,wen_toward_2021,von_kugelgen_self-supervised_2021,saunshi_understanding_2022}, a conceptual framework for comparing and deriving any future ISSL method is still missing.
Indeed, most previous theory \cite{lee_predicting_2020,saunshi_theoretical_2019,tosh_contrastive_2021,bansal_for_2020,nozawa_pac-bayesian_2020,bao_sharp_2021} prove that specific class of methods are \textit{sufficient} to learn useful representations. 
\ydnote{We really have to rephrase people will be critical / defensive.}
Instead, our desired framework should characterize \textit{all} desired representation through sufficient and \textit{necessary} requirements.
Such a goal is hard with theoretical tools that aim at providing bounds that hold in practice.
In this paper, we drop the latter requirement and instead analyze optimal ISSL representation.
As a result, we derive s theoretical framework to analyze, improve, and derive any future ISSL methods by providing necessary and sufficient requirements which then have to be approximated in practice.

Specifically, we characterize all encoders that ensure that downstream specific predictors (\eg linear or MLP) can achieve the Bayes risk on any task that is invariant to desired transformation (\eg data augmentations).
Essentially, we prove that the task information is in the representation and usable by desired predictors if and only if predictors can :
\begin{inlinelist}
\item separate positive (equivalent) and negative (non-equivalent) examples from the representation; and
\item shatter the representations.
\end{inlinelist}
\ydnote{
This summary should be intuitive, but I don't think shattering is intuitive. 
}
\ydimp{
Need a nice figure 1, but not sure which! \percy{} ?
}

Based on our theory we derive prescriptive insights into ISSL, \eg, how to chose the: augmentations, dimensionality of the representation, regularizers, or ISSL objective.
For example, we show that existing ISSL tricks and objectives are various (suboptimal) approximations to the two aforementioned requirements. 
By modifying those approximations we experimentally improve existing methods on standard benchmarks. In summary we:
\ydnote{extend experimental section once know exactly the results}
\begin{itemize}[noitemsep]
\item prove minimal and sufficient requirements to solve any invariant task using desired predictors.
\item provide insights into ISSL which allows us to improve existing methods on (Tiny)ImageNet.
\end{itemize}

==> text/problem_old.tex <==
\ydnote{I'm counting on the fact that we have the loss decomposition paper on arxive before or at the same time as this one}
Following \tocite{}, we refer to SSL as \textit{learning representations} $\rv Z$ of inputs $\rv X$ that are useful for a set of downstream supervised tasks $\tasks{}$ that are only \textit{partially} known during representations learning.

\subsection{Representation learning : discriminativeness and sample efficiency}
\label{subsec:problem_rep}

In practical SSL, representation learning consists of training an encoder $\p{Z|X}$, which will be evaluated using the accuracy of a constrained predictive family $\Q$, \eg, linear or multi-layer perceptron (MLP), on a set of classification tasks $\tasks{}$.
Potential task $\tasks{} \defeq \set{Y_{dog}, Y_{geo}, \dots}$ might include linearly predicting the presence of a dog $\rv Y_{dog}$ or the country in which a picture was taken $\rv Y_{geo}$. 

One thus wants a representation $\rv Z$ which ensures that, on \textit{any} downstream task $\rv Y \in \tasks{}$, the best performance is as high as possible.
This suggests minimizing the \textit{worst-case excess Bayes risk}, 
%
\begin{equation}\label{eq:worst_case}
\distsT{} \defeq 
\sup_{\footnotesize Y \in \tasks{}} \quad \RiskA{Y}{Z} - \RiskU{Y}{X},
\end{equation}
%
where $\Risk{\rv Y}{\rv Z} \defeq \inf_{\pred{} \in \Q} \Ep{\p{Y,X}\p{Z|X}}{\indneq{\rv Y}{\pred{}(  \rv Z))}}$ is the Bayes risk (best possible 0-1 loss) when using constrained predictors $\Q$ from the representation's space $\Zc$, while $\U$ are unconstrained predictors from the input's space $\Xc$. We call encoders that minimize \cref{eq:worst_case} \textit{discriminative} for $\tasks{},\Q$.

Discriminativeness concerns the existence of constrained predictors that performs as well as possible on tasks in $\tasks{}$. 
In practice, we additionally want such predictors to be recoverable using standard empirical risk minimization (ERM) on the least amount of downstream samples. 
We will call representations that ensure such property \textit{sample efficient}, but postpone that discussion to \cref{sec:sample_efficiency}.

\subsection{Invariant self-supervised learning (ISSL)}

In SSL we cannot directly optimize \cref{eq:worst_case} as we do not know all desired tasks $\tasks{}$.
Typically, practitioners have partial knowledge of $\tasks{}$, which they incorporate using transformations that intuitively preserve downstream target.
For image classification, one can use standard augmentations, \eg random cropping, or more complex transformations such as image-to-text pairing \cite{radford_learning_2021}.
In both cases practitioner tell the model that some ``positive'' examples are equivalent $x \sim x^+$ for tasks of interest.

We formalize this using an equivalence relation $\sim$ on $\Xc$ that preserves the most likely label.
In other words, $\sim$ induces a partition of inputs $\mathcal{X}$ into \textit{equivalent classes}, and we consider tasks $\tasksinv{}$ whose most likely labeling is constant within these classes.
This is more general than the typical 
\cite{leen_data_1994,chen_group-theoretic_2020,lyle_benefits_2020} group theoretical formalization of augmentations: augmentations can be example dependent (\eg the digit ``3'' is invariant to $\pi$ rotations but ``6'' is only invariant to $\frac{\pi}{2}$) and do not have to be invertible (\eg cropping).
We refer to SSL for $\tasksinv{}$ as \textit{invariant SSL} (ISSL).
\ydnote{
In practice you will likely be interested in only a subset of this task sets. 
In that case we should use fuzzy equivalence relations. But that's for future paper(s).
}
%
\begin{definition}\label{def:inv_task}
The set of
\textit{invariant tasks}
\footnote{
This extends \citepos{dubois_lossy_2021} invariant tasks to cases where the label conditional distribution change. 
}
$\tasksinv{}$ with respect to an equivalence $(\mathcal{X},\sim)$, is all random variables $\rv Y$ s.t. 
$x \sim x^+ \implies \argmax_{y \in \Yc} p(y|x) = \argmax_{y \in \Yc} p(y | x^+)$ for any $x,x^+ \in \Xc$.
\end{definition}





%We generalize our results to uncountable spaces in \toappx{}, but note that the finite setting holds in practice due to finite computations.
% \ydnote{ I prefer avoiding measure theory in main paper, and keep it for appcs. 
% Also we might have to assume finite $M(X)$ in any case (although maybe not, I need to double check).
% }
%For the encoders $\mathcal{E}$, we make no assumptions on the sample space $\mathcal{Z}$ (\eg dimensionality of $\rv Z$) and stochastic encoders, but assume that $\mathcal{E}$ contains all deterministic functions from $\mathcal{X}$ to $\mathcal{Z}$.
%In the main paper, we only consider the population risk as downstream predictors $\Q$ generalize well in practice \tocite{}, likely due to their simplicity (linear or shallow MLP).
%We deal with empirical risks in \toappx{}.

% For clarity we will first consider the standard setting of classification with accuracy loss $\ell(y, f(z)) = \indeq{y}{f(z)}$, and representation space $\mathcal{Z} \subseteq \mathbb{R}^d$ for some $d$.
% We generalize different losses in \tocref{}, and drop any superscripts $\ell$ until then.
% The most likely label is then denoted as $\bayesA{Y|X} (x) \defeq \argmax_{y \in \mathcal{Y}} p(y | x)$.
%, where ${ \scriptstyle \%}$ is a shorthand for accuracy.
% To improve clarity in the main paper, we also assume that all sample spaces are finite (albeit arbitrarily large), \eg, real numbers with finite precision.
% We generalize our results to uncountable spaces in \toappx{}, but note that the finite setting holds in practice due to finite computations.
% \ydnote{ I prefer avoiding measure theory in main paper, and keep it for appcs. 
% Also we might have to assume finite $M(X)$ in any case (although maybe not, I need to double check).
% }
%\textit{meaningful} \cite{dubois_lossy_2021} point-wise loss functions $L$, namely functions that are minimized if and only if the predictions are exact $f(z)=y$. \ydnote{might have to restrict oursleves to accuracy} For example squared error or accuracy.



==> text/short_conclusion.tex <==
\label{sec:discussion}


We presented a simple conceptual framework to understand, compare and improve ISSL methods.
Inspired by recent work on optimal representations for supervised \cite{dubois_learning_2020} and robust \cite{ruan_optimal_2022} learning, we derived such a framework by studying   algorithmic-agnostic goals for ISSL.
In particular, \cref{thm:main} provides the minimal and sufficient requirements for optimal encoders.
%, and \cref{prop:coupon} gives the resulting probing risk as a function of pretraining augmentations. 
On the algorithmic side, 
\cref{sec:approximations} uses our framework to derive simpler and theoretically-motivated variants of prior SSL objectives.
Altogether our framework provides actionable insights for ISSL such as how to choose: SSL algorithms, the dimensionality of the representations, projection heads, and augmentations.
On the empirical side, \cref{sec:experiments} shows that our prescriptions leads to significant gains
%.Our final SSL algorithms outperform strong baselines (SwAV+multicrop trained on ImageNet) 
on linear probing benchmarks.\looseness=-1

There are many limitations that should be addressed for a more realistic prescriptive framework for ISSL.
See \cref{sec:appx:discussion} for more details.
First, our theory is binary, \eg,  augmentations are either label preserving or not, and encoders are optimal or not. 
Although our framework likely captures the right intuition, nuance would be more realistic. 
Second, we consider unconstrained encoders $\enc{}$, \iupdated{dimensionality}, and infinite unlabeled data.
As a result, our framework cannot currently improve the computational or data efficiency of the pretraining phase.
Finally, we consider all invariant tasks $\tasksinv{}$ even though only a subset of those are meaningful.
%Optimal representations for this subset will be different, and defining this subset likely requires considering inductive biases of encoders \cite{saunshi_understanding_2022}.
Despite those limitations, we 
showed that our framework's insights lead to substantial improvements in ISSL performance.\looseness=-1



==> text/theory_old.tex <==
In this section we provide minimal and sufficient requirement for discriminative and sample efficient encoders in ISSL.
For simplicity, our presentation is relatively informal; formal proofs are in \cref{sec:appx:proofs}.
% We assume that $\Q$ contains at least linear predictors, and that the $\inf$ is taken only over those that are well defined (correct domain and codomain).
% For example $\Q$ could be the set of MLPs with a specific architecture trained with gradient descent.\footnote{The width of hidden layers should at least $ \min(|\mathcal{Z}|,|\mathcal{Y}|)$ to contain all linear predictors.}
% In case the family is unconstrained (universal) we will denote it as $\Q=\U$.
In the main paper we assume that downstream predictors $\Q$ include at the set of linear predictors.
For clarity, we also assume that sample spaces are finite, \eg, finite precision floats.

\ydnote{Generalization to uncountable $Z,X$ with finite number of equivalence classes should not be too hard. I honestly don't care much as everything is finite on computers.
}

\subsection{Discriminativeness}
\label{sec:decodability}
\input{text/decodability}

\subsection{Sample efficiency}
\label{sec:sample_efficiency}
\input{text/sample}
